Non-Malleable Codes for Small-Depth Circuits

We construct efficient, unconditional non-malleable codes that are secure against tampering functions computed by small-depth circuits. For constant-depth circuits of polynomial size (i.e. $\mathsf{AC^0}$ tampering functions), our codes have codeword length $n = k^{1+o(1)}$ for a $k$-bit message. This is an exponential improvement of the previous best construction due to Chattopadhyay and Li (STOC 2017), which had codeword length $2^{O(\sqrt{k})}$. Our construction remains efficient for circuit depths as large as $\Theta(\log(n)/\log\log(n))$ (indeed, our codeword length remains $n\leq k^{1+\epsilon})$, and extending our result beyond this would require separating $\mathsf{P}$ from $\mathsf{NC^1}$. We obtain our codes via a new efficient non-malleable reduction from small-depth tampering to split-state tampering. A novel aspect of our work is the incorporation of techniques from unconditional derandomization into the framework of non-malleable reductions. In particular, a key ingredient in our analysis is a recent pseudorandom switching lemma of Trevisan and Xue (CCC 2013), a derandomization of the influential switching lemma from circuit complexity; the randomness-efficiency of this switching lemma translates into the rate-efficiency of our codes via our non-malleable reduction.

==> ingredients.tex <==
\iffalse
\subsection{A ``Leakage-Tolarant'' Non-malleable Code against Local Tampering}
\mbnote{Best Split-State NMC Theorem}

See Section~\ref{sec:bdkm+}
\begin{theorem}[\cite{BDKM16}]
	\label{thm:bdkm+}
	For $\ell(n)=o(n/\log n)$,
	there exists a $(\Local^\ell\implies\textsc{SS},\negl(n))$-non-malleable reduction, $(\E'_\ell,\D'_\ell)$, such that $\E:\zo^{2k}\to\zo^n$ and $n=O(\ell(n)k)$.
	
	Moreover, $(\E'_\ell,\D'_\ell)$ is a $(\leaky_\star^{\ell',\delta,B}\implies \textsc{SS})$-non-malleable reduction.
	\mbnote{parameters?}
\end{theorem}
\mbnote{maybe restate using normal rate terminology?}
\sgnote{suggest to state using $\leaky^{d,m,k}[\Local^{k^\delta}]$ instead of $\leaky_\star^{\ell',\delta,B}$}

\begin{corollary}
	\label{cor:bdkm16}
	For all $\varepsilon<1$
	and $\ell(n)=O(n^\varepsilon)$,
	there is a non-malleable code $(\E_\ell,\D_\ell)$ against $\leaky^{\ell',\delta,B}$ tampering with rate polynomial rate, XXXX.
\end{corollary}
\sgnote{I comment this out because we don't need this for the non-malleable reduction and we will revisit it in the last section.}
\fi	

\subsection{A Binary Reconstructible Probabilistic Encoding Scheme}
Reconstructable Probabilistic Encoding (RPE) schemes were first introduced by Choi et al.~\cite{CDMW08, CDMW16}. Informally, RPE is a combination of error correcting code and secret sharing, in particular, it is an error correcting code with an additional secrecy property and reconstruction property.
\begin{definition}[Binary Reconstructable Probabilistic Encoding] 
	\cite{CDMW08,CDMW16}
	We say a triple $(\E, \D, \R)$ is a {\sf binary reconstructable probabilistic
		encoding scheme} with parameters $(k, n, \cerr, \csec)$, where
	$k, n \in \bbN$, $0 \leq \cerr,\csec < 1$, if it
	satisfies the following properties: 
	
	\begin{enumerate}
		\item \textbf{Error correction.} 
		$\E\colon \zo^k \rightarrow \zo^n$ is an efficient probabilistic
		procedure, which maps a message $x \in \zo^k$ to a distribution over
		$\zo^n$. If we let $\cC$ denote the support of $\E$, any two
		strings in $\cC$ are $2\cerr$-far.
		Moreover, $\D$ is an efficient procedure that
		given any $w' \in \zo^n$ that is $\epsilon$-close to some string $w$ in
		$\cC$ for any $\epsilon \leq \cerr$, outputs $w$ along with a consistent $x$.
		\item \textbf{Secrecy of partial views.} 
		For all $x \in \zo^k$ and any non-empty set $S \subset [n]$ of size $\leq \lfloor\csec\cdot n\rfloor$, $\E(x)_S$ is
		identically distributed to the uniform distribution over $\zo^{|S|}$.  

		
		\item \textbf{Reconstruction from partial views.} 
		$\R$ is an efficient procedure that given any set $S \subset [n]$ of size $\leq \lfloor\csec\cdot n\rfloor$,
		any $\hat{c} \in \zo^n$, and any $x \in \zo^k$, samples
		from the distribution $\E(x)$ with the constraint  $\E(x)_S={\hat{c}}_S$.  
	\end{enumerate}
\end{definition}

\begin{lemma} \cite{CDMW08,CDMW16}%thm 2.1
	\label{lem:rpe}
	For any $k \in \bbN$,
	there exist constants $0<\crate,\cerr,\csec<1$ such that
	there is a binary RPE scheme with parameters
	$(k, \crate k, \cerr, \csec)$.
\end{lemma}

%	\dnote{Sometimes we want our RPE to expand beyond constant times $k$ (e.g. in Section 5). Copying the following from BDKM16:}  \sgnote{got it}

To achieve longer encoding lengths $n$, with the same $\cerr,\csec$  parameters, one can simply pad the message to an appropriate length.  

RPE has been used in Ball et al.\cite{BDKM16} for building non-malleable reduction from local functions to split state functions.  However, for all reductions in our paper, RPE without error correction property suffices. In addition, we observe that RPE with paremeters $(k,n,0,\csec)$ is implied by any linear error correcting code with parameters $(k,n,d)$ where $k$ is the message length, $n$ is the codeword length, $d:=\csec\cdot n+1$ is the minimal distance. 

\begin{lemma}\label{lm:wRPE}
Suppose there exists a binary linear error correcting code with paremeters $(k,n,d)$, then there is a binary RPE scheme with parameters $(k,n,0,(d-1)/n)$.
\end{lemma}


\begin{proof}
For a linear error correcting code with $(k,n,d)$,  let $A$ denote its encoding  matrix, $B$ denote its decoding matrice, $H$ denote its parity check matrix. Note that by the decoding property, $BA=I$, by property of parity check matrix, $HA=\bold{0}$ and $Hs\neq 0$ for any $0< ||s||_0<d$ where $I$ is  the $k\times k$ identity matrix, $\bold{0}$ is the $(n-k)\times k$ all $0$ matrix.

We define $(\E,\D,\R)$ as follows: for $x\in\zo^k$ and randomness $r\in\zo^{n-k}$, $\E(x;r):=B^Tx+H^Tr$, for $c\in\zo^{n}$; $\D(c):=A^Tc$; given $S \subset [n]$ of size $\leq d-1$ , $\hat{c} \in \zo^n$,  $x \in \zo^k$, $\R$ samples $r$ uniformly from the solutions to $(H^Tr)_S=(\hat{c}-B^Tx)_S$ then outputs $\E(x;r)$. 

$(\E,\D)$ is a coding scheme because  $\D\circ\E =A^TB^T=I^T=I$.  For secrecy property, note that for any non-empty $S\subseteq[n]$ of size at most $d-1$, $(Hr)_S$ distributes uniformly over $\zo^{|S|}$, because for any $a\in\zo^{|S|}$, \[\Pr_{r}[(H^Tr)_S=a]=\E[\Pi_{i\in S}\frac{1+(-1)^{(H^Tr)_i+a_i}}{2}]=2^{-|S|}\sum_{S'\subseteq S} \E[\Pi_{i\in S'}(-1)^{(H^Tr)_i+a_i}]=2^{-|S|},\]
where the last equality is because the only surving term is $S'=\emptyset$ and for other $S'$, $\sum_{i\in S'}H^T_i\neq 0$ so $\E[\Pi_{i\in S'}(-1)^{(H^Tr)_i}]=0$.
It implies $\E(x)_S$ also distributes uniformly  over $\zo^{S}$. By definition, $R$ satisfies reconstruction property.  Hence $(\E,\D,\R)$ is a binary RPE with parameters $(k,n,0,(d-1)/n)$.

\end{proof}





\subsection{A Simple $q$-wise Independent Generator}

\begin{definition} [Bounded-independent Generator] We say a distribution $\mathcal{D}$ over $\zo^n$ is {\em $q$-wise independent} if for any $S\subseteq [n]$ of size at most $q$, $\mathcal{D}_S$ distributes identically to the uniform distribution over $\zo^{|S|}$. We say function $G\colon\zo^s\rightarrow\zo^n$ is a $q$-wise independent generator if $G(\zeta)$ is $q$-wise independent where $\zeta$ is uniformly distributed over $\zo^s$.	
\end{definition}

%\mbnote{move to appendix}
%\mbnote{may be missing some constants.}
The simple Carter-Wegman hashing construction based on random polynomials suffices for our purposes.
\begin{lemma}
	\label{lem:gen}
	\cite{CW81}
	There exists an (explicit) $q$-wise independent generator:
	$G:\zo^{(q+1)\log n}\to\zo^{n}$, computable in time $\tilde{O}(qn)$.
	
	Moreover, $G:\zo^{(q+1)m}$ can be constructed such that for an subset $S\subseteq[n]$ of size $q$, $G(\zeta)_S \equiv X_1,\ldots,X_q$ (for uniformly chosen $\zeta$) where (1) $X_i$'s are independent Bernoullis with $\Pr[X_i=1]=q/d$ for $q\in\{0,\ldots,d\}$, and (2) $m=\max\{\log n,\log d\}$.
\end{lemma}

Let $G_{q,p}$ denote a $q$-wise independent Carter-Wegman generator with bias $p$, and $G_{q}$ such a generator with $p=1/2$

The following useful theorem gives Chernoff-type concentration bounds for $q$-wise independece distributions. %(not to mention the previous section).
\begin{theorem}[\cite{SSS95}]
	\label{thm:pr-chernoff}
	If $X$ is a sum of $q$-wise independent random indicator variables with $\mu=\bbE[X]$, then $\forall\ 0<\varepsilon\leq1,q\leq\varepsilon^2\mu e^{-1/3}$, 
		$\Pr[|X-\mu|>\varepsilon\mu] < \exp(-\lfloor q/2 \rfloor)$.
%		\forall\ 0<\varepsilon\leq1,q\leq\lfloor\varepsilon^2\mu e^{-1/3}\rfloor\]
%		
%	\begin{align*}
%		\Pr[|X-\mu|>\varepsilon\mu] &< \exp(-\lfloor q/2 \rfloor)
%		&\forall\ 0<\varepsilon\leq1,q\leq\lfloor\varepsilon^2\mu e^{-1/3}\rfloor\\
%		\Pr[|X-\mu|>\varepsilon\mu] &< \exp(-\lfloor \varepsilon^2\mu/3 \rfloor)
%		&\forall\ 0<\varepsilon\leq1,q\geq\lfloor\varepsilon^2\mu e^{-1/3}\rfloor\\
%		\Pr[|X-\mu|>\varepsilon\mu] &< \exp(-\lfloor q/2 \rfloor)
%		&\forall\varepsilon\geq1,q\leq\lfloor\varepsilon^2\mu e^{-1/3}\rfloor\\
%		\Pr[|X-\mu|>\varepsilon\mu] &< \exp(-\lfloor \varepsilon\mu/3 \rfloor)
%		&\forall\varepsilon\geq1,q\geq\lfloor\varepsilon^2\mu e^{-1/3}\rfloor\\
%		\Pr[|X-\mu|>\varepsilon\mu] &< \exp(-\varepsilon\ln(1+\varepsilon)\mu/2)
%		&\forall\varepsilon\geq1,q\geq\lceil\epsilon\mu\rceil
%	\end{align*}
\end{theorem}	

\subsection{A Pseudorandom Switching Lemma}
\begin{definition}
	\label{def:enc-prr}
	Fix $p\in(0,1)$.
	A string $s\in\zo^{n\times \log(1/p)}$ encodes a subset 
	$L(s)\subseteq[n]$ as follows:
	for each $i\in[n]$,
	\[ i\in L(s) \iff s_{i,1}=\cdots=s_{i,\log(1/p)}=1.\]
\end{definition}

\begin{definition}
	\label{def:prr}
	Let $\cD$ be a distribution over $\zo^{n\log(1/p)}\times\zo^n$.
	This distribution defines a distribution $\cR(\cD)$ over restrictions $\{0,1,*\}^n$,
	where a draw $\rho\gets\cR(\cD)$ is sampled as follows:
	\begin{enumerate}
		\item Sample $(s,y)\gets \cR(\cD)$,
		where $s\in\zo^{n\log(1/p)},y\in\zo^n$.
		\item Output $\rho$ where
		\begin{align*}
			\rho_i := \left\{
			\begin{array}{rl}
				y_i &\mbox{if } i\notin L(s)\\
				* &\mbox{otherwise}
			\end{array}
			\right.
		\end{align*}
	\end{enumerate}
\end{definition}

The following is a simple corollary of the pseudorandom switching lemma in~\cite{TX13}.

\iffalse
\begin{lemma}[Pseudorandom Switching Lemma]
	\label{lem:psl}
	\cite{TX13}
	
	Fix $(p,\delta)\in(0,1)$ and $w,\ell\in\bbN$.
	Then, there exists a value $r\in\bbN$,
	\[r=\poly(\log \ell, w,\log(1/\delta),\log n)\]
	such that the following holds.
	
	Let $\cD$ be any $r$-wise independent distribution over $\zo^{n\log(1/p)}\times\zo^n$.
	Let $F_1,\ldots,F_M$ be $M$ many width-$w$ DNFs,
	then
	\[\Pr_{\rho\gets\cR(\cD)}\left[\exists j\in[M]\mbox{ such that $(F_j\upharpoonright\rho)$ is not $\ell-\Local$}\right]
	\leq M\left(2^{w+\log\ell+1}(5pw)^{\log \ell}+ \delta\right)\]
\end{lemma}
\fi

\begin{lemma}[Pseudorandom Switching Lemma]
	\label{lem:psl}
	\cite{TX13}
	
	Fix $(p,\delta)\in(0,1)$ and $w,S,t\in\bbN$.
	Then, there exists a value $r\in\bbN$,
	\[r=\poly(t, w,\log(S),\log(1/\delta),\log(1/p))\footnote{The exponent of this polynomial is a fixed absolute constant independent of all other paramemters.}\]
	such that the following holds.
	
	Let $\cD$ be any $r$-wise independent distribution over $\zo^{n\log(1/p)}\times\zo^n$.
	Let $F=F_1,\ldots,F_M$ where $F_1,\dots,F_M$ are size-$S$ depth-$2$ circuits with bottom fan-in $w$,
	then
	\[\Pr_{\rho\gets\cR(\cD)}\left[F_\rho\text{ is not in }\DT(t)\right]
	\leq M\left(2^{w+\log\ell+1}(5pw)^{\log \ell}+ \delta\right).\]
\end{lemma}


Lastly, we define some convient functions. For a random restriction  $\rho=(\rho^{(1)},\rho^{(2)})\in\{0,1\}^{n}\times\zo^{n}$, $\extInd(\rho^{(1)}):=(i_1,\ldots,i_k)\in [n+1]^k$ are the last $k$ indices of 1s in $\rho^{(1)}$ where $i_1\leq i_2\dots\leq i_k$ and $i_j=n+1$ for $j\in[k]$ if such index doesn't exist ($k$ should be obvious from context unless otherwise noted).  

We define a pair of functions for embedding and extracting a string $x$  according to a random restriction, $\rho$. Let $\embed:\zo^{k+2n}\to\zo^n$, $\extract:\zo^{2n}\to\zo^k\times\{\bot\}$
such that
\begin{itemize}
	\item[] for $\rho=(\rho^{(1)},\rho^{(2)})\in\{0,1\}^{n}\times\zo^{n}$ and $x\in\{0,1\}^k$, and $i\in[n]$,
	
	%\\ if $i=\extInd(\rho^{(1)})_j$ for some $j\in[k]$ then $\embed(x,\rho)_i:= x_j$ otherwise $\embed(x,\rho)_i:= x_j$.
	\begin{equation*}
		\embed(x,\rho)_i = 
		\left\{\begin{array}{rl}
			x_j & \mbox{if } \exists j\in[k], i=\extInd(\rho^{(1)})_j \\
			\rho_i^{(2)} & \mbox{otherwise}\\
		\end{array}\right.
	\end{equation*}
	\item[] if $c\in\zo^n,\rho^{(1)}\in\{0,1\}^n$, and $\|\rho^{(1)}\|_0\geq k$,
	then 
	\begin{equation*}
		\extract(c,\rho^{(1)})=c_{\extInd(\rho^{(1)})}. 
	\end{equation*}
	Otherwise, $\extract(c,\rho^{(1)})=\bot$.
\end{itemize}

Note that, for any $\rho$ of $\|\rho^{(1)}\|_0\geq k$,
\[ \extract(\embed(x,(\rho^{(1)},\rho^{(2)})),\rho^{(1)})=x.\]	
\iffalse		
\begin{proposition}
	\label{prop:width}
	For $q>w$,
	the probability a size $S$ $\dnf$ have width more than $w$ under a pseudorandom restriction with $p\leq1/2$ is at most $S(2^{\log(3/4)w})$.
\end{proposition}
\begin{proof}
	Let $T$ be a term of width $w'>w$.
	Recall that $p=1/2$.
	Therefore, probability that $(T|\rho)$ is not constant is at most $(3/4)^{w}$, by the independence properties of $G$.
	Finally, union bounding over all $S$ possible terms yields the claim.
\end{proof}

\subsection{Helpful functions.}
\fi	




==> leaky-analysis.tex <==
In this section, we compose the basic non-malleable reduction $(\E^\star,\D^\star)$ and prove our main results. 

\begin{theorem} \label{thm:ac0}
Let $n\in\mathbb{N}$ and $c\in(0,1)$ be a constant. There exists a constant $C\geq 1$ such that for any $d\leq\log{n}/(C\log\log{n})$, $S=\poly(n)$, there exist $p,\sigma$ and $n_1\leq\dots\leq n_{d-1}\in\mathbb{N}$, so that %$(\E_{k,n_1,p,q}^\star\circ\cdots\circ\E_{n_{d-1},n,p,q}^{\star},\D_{k,n_1,p,q}^\star\circ\cdots\circ\D_{n_{d-1},n,p,q}^\star)$
 $(\E_{n_{d-1},n}^\star\circ\cdots\circ\E_{k,n_1}^{\star}\ , \D_{k,n_1}^\star\circ\cdots\circ\D_{n_{d-1},n}^\star)$
%			$(\underbrace{\E_{q,p,n}^\star\circ\cdots\circ\E_{q,p,n_1}^\star}_{\times d},\underbrace{\D_{q,p,n}^\star\circ\cdots\circ\D_{q,p,n_1}^\star}_{\times d})$
		is an $(\AC_d(S)\implies\leaky^{d,m,n}[\Local^{k^c}],d\varepsilon)$-non-malleable-reduction with rate $\big(O(\log^{-2}n)\big)^{d}$, where  $\varepsilon=n^{-\Omega(\log\log{n})}$, $m=\poly\log(n)$.
\end{theorem}

Note that for constant depth circuit, $n$ is quasilinear in $k$. Moreover even for $d$ being as large as  $\Omega(\log n/\log\log{n})$, $n$ is $k^{1+\delta}$ for a small constant $\delta<1$. 
\mbnote{This is disingenuous for us to note, suggests we can get an NMC for $\AC$ with rate $\Omega(1/\log^{O(1)k})$. Unfortunately, for $p^{-1}=\log^{O(1)}n$ we need $\log\ell = \omega(\log n/\log\log n)$. However, for the Local NMC to have rate $1/\poly\log$, we need $\ell = O(\log^{O(1)}n) \implies \log \ell = O(\log\log n)$.} 
By combining with the non-malleable code for leaky local functions from Lemma~\ref{lem:local-nmc}, we obtain the following result.




\begin{corollary}
	\label{cor:main}
	For any constant $0<\delta<1$, there exists a sufficiently large constant $C\geq 1$ so that for any $d\leq\log{n}/(C\log\log{n})$  and $S=\poly(n)$, there is an explicit, efficient, information theoretic $(\AC_d(S),\negl(n))$-non-malleable code with rate $n=O(k^{1+\delta})$.
	
	%k^{1+\delta}=n \iff n^{1/(1+\delta)}=k
	%\iff 1/(1+\delta) = 1-2\eps
	%\iff 1 = (1-2\eps)(1+\delta)
	%\iff 1 = 1 - 2\eps +\delta -2\eps\delta
	%\iff \delta = 2\eps(1+\delta)
	%\iff \eps = \delta/(2+2\delta)
	%and then an extra factor of log k, handle by shaving exponent
\end{corollary}

\mbnote{I'm losing my mind right now, but can get error (and, 1/size) bound up to $n^{\Omega(\log n)}$ and can (composed rate) to such that $n=O(k^{1+o(1)})$, but the tradeoffs with depth and error are a bit tricky. Will update soon}

Our main lemma shows we can  use the basic reduction to trade depth for leakage.

\begin{lemma}
		\label{thm:red}
		Let $i,w,t,d,S,W,S',N\in\bbN$ and $\delta\in(0,1)$. For 
		$n,k,p,\sigma$ satisfying constraints in Figure~\ref{fig:red} 
		and $\sigma= r(t,w,\log(S'),\log(1/\delta),\log(1/p))$.  
		$(\E^\star,\D^\star)$ is an ($\leaky^{i,m,N}[\AC_d(S,W)\circ w\text{-}\AC_2(S')]\implies \leaky^{i+1,m,N}[\AC_{d}(S,W)\circ\DT(t)],\varepsilon$)-non-malleable reduction where  $\varepsilon=\exp(-\Omega(\sigma/\log{1/p})) + NW\left(2^{w+t+1}(5pw)^{t}+ \delta\right)$ and $m=O(\sigma\log{n})$.
\end{lemma}
The proof of Lemma~\ref{thm:red} is a straightforward generalization of the proof of Proposition~\ref{prop:psl-nmr}. We first prove our main theorem given Lemma~\ref{thm:red}.

\begin{proof} [Proof of Theorem~\ref{thm:ac0}]
Let $w:=\log{n}$, $t:=c\log{k}$, $\delta:=n^{-\log\log{n}}$, $p:=1/\log^2{n}$ and $\sigma:=r(t,w,\log(S+d\cdot 2^t),\log(1/\delta),\log(1/p))=\poly\log(n)$.

Note that because $t<w$ and any depth $t$-decision tree can be computed by width-$t$ DNFs or width-$t$ CNFs of size $2^t$, for any $d,S\in\bbN$, $\AC_{d'}(S,W)\circ\DT(t)$ is a subclass of $\AC_{d'-1}(S,W)\circ w\text{-}\AC_2(W2^t)$. Combining Lemma~\ref{thm:red} and the fact that $\AC_d(S,W)\subseteq1\text{-}\AC_{d+1}(S,W)$, $(\E_{n_{d-1},n}^\star,\D_{n_{d-1},n}^\star)$ reduces $\AC_d(S,W)$ to $\leaky^{1,m,n}[\AC_{d-2}(S,W)\circ w\text{-}\AC_2(W\cdot2^t)]$ with error $\varepsilon=\exp(-\Omega(\sigma/\log{1/p})) + n\left(2^{w+t+1}(5pw)^{t}+ \delta\right)$. 

For $2\leq i\leq d-1$,  by Lemma~\ref{thm:red} and $\DT(t)\subseteq w$-$\AC_{2}(2^t)$,  $(\E_{n_{d-i},n_{d-i+1}}^\star,\D_{n_{d-i},n_{d-i+1}}^\star)$ reduces 
 $(\leaky^{i-1,m,n}[\AC_{d-i}(S,W)\circ w\text{-}\AC_2(W2^t)]$ to $\leaky^{i,m,n}[\AC_{d-i-1}(S,W)\circ w\text{-}\AC_2(W2^t)]$
with error at most $\varepsilon$.  Finally, by Lemma~\ref{thm:red} and the fact $\DT(t)$ is a subclass of $\Local^{2^t}$, $(\E_{k,n_1}^\star,\D_{k,n_1}^\star)$ reduces 
$\leaky^{d-1,m,n}[w\text{-}\AC_{2}(W2^t)]$ to $\leaky^{d,m,n}[\Local^{2^t}]$ with error at most $\varepsilon$.  Therefore $(\E_{n_{d-1},n}^\star\circ\cdots\circ\E_{k,n_1}^{\star}\ , \D_{k,n_1}^\star\circ\cdots\circ\D_{n_{d-1},n}^\star)$ reduces $\AC_d(S,W)$ to $\leaky^{d,m,n}[\Local^{2^t}]$ with error at most $d\varepsilon$.

Note that the rate of the code is $(O(p))^d$ and $\log k=\log n - d\log(O(p))=\Omega(\log{n})$ for $d\leq\log{n}/(C\log\log{n})$ for a sufficiently large $C$ (depending only on $c$). Hence $n(2^{w+t+1}(5pw)^{t}) = 2n^2(10/\log{n})^{c\log k} = n^{-\Omega(\log\log{n})}$. 
In addition, because $\exp(-\Omega(\frac{\sigma}{\log(1/p)}))+n\cdot\delta=n^{-\Omega(\log\log{n})}$ by our choice of $\delta$ and $\sigma$, we conclude $\varepsilon=n^{-\Omega(\log\log{n})}$. 

\iffalse 
We get that (ii) $(\E_{\sigma,p,n}^\star,\D_{\sigma,p,n}^\star)$ is a ($[\AC_d(S)]\implies \leaky^{1,m,n}[w-\AC_{d}(S')],\varepsilon$)-non-malleable reduction, where $\varepsilon=?$ and $S'=S2^t$.


 Combining with Lemma~\ref{thm:red}, we have that for any $i\leq d$ and $n'\leq n$, (i)
		$(\E_{q,p,n'}^\star,\D_{q,p,n'}^\star)$ is a ($\leaky^{i,m,n}[w-\AC_d(S)]\implies \leaky^{i+1,m,n}[w-\AC_{d-1}(S')],\varepsilon$)-non-malleable reduction,
		where $\varepsilon=\exp(-\Omega(\frac{q}{\log(1/p)})) + n\left(2^{w+t+1}(5pw)^{t}+ \delta\right)$.
Additionally, if we consider $\vF\in\AC_d(S)$ to have an additional layer of fan-in 1 AND/OR gates, we get that (ii) $(\E_{q,p,n}^\star,\D_{q,p,n}^\star)$ is a ($[\AC_d(S)]\implies \leaky^{1,m,n}[w-\AC_{d}(S')],\varepsilon$)-non-malleable reduction, where $\varepsilon=?$ and $S'=S2^t$.
Combining (i) and many $d$ applications of (ii) and the fact that $\AC_0\circ\DT(t)=\DT(t)\subseteq\Local^{2^t}$,
we get our main theorem.
\fi
\end{proof}
	\begin{figure}[ht!]
		\fbox{\parbox{\textwidth}{
				
				\small \center
				\begin{minipage}{0.95\textwidth}
					given $\leaky^{i,m,N}[\AC_d(S,W)\circ w\text{-}\AC_2(S')]$ tampering $\tau=(\vF,h_1,\ldots,h_i)$ output $\tau'=(\vF',h'_1,\ldots,h'_{i+1})$:
					\begin{enumerate}
						\item Draw (uniformly) random seed $\zeta\gets\{0,1\}^s$ 
						and (uniformly) random string $R\gets\{0,1\}^{n-m}$.
						
						\item Generate pseudorandom restriction, $\rho=(\rho^{(1)},\rho^{(2)})$:
						\begin{itemize}
							\item[] $\rho^{(1)} \gets L(G(\zeta))$. ($*$) If $\|L(G(\zeta))_{n-m+1,\ldots,n}\|_0< k$, set $\zeta=\zeta^{*}$.  
							%			($*$) If the index of the $k$-th 1 in $L(G(\zeta))$ is $\leq n-m$
							%			(or does not exist), 
							%			use some fixed $\zeta^*$ such that
							%			$\|L(G(\zeta^*))_{n-m+1,\ldots,n}\|_0\geq k$.
							%			\mbnote{$k$ is overloaded}
							%			(For $G$ from Lemma~\ref{lem:gen} such a $\zeta'$ can be found
							%			via interpolation in time $O(q\log^2n)$.)
							%		
							\item[] $\rho^{(2)} \gets \E_R(\zeta)\|R$
						\end{itemize}
						\item Apply (constructive) switching lemma with pseudorandom restriction to get $\AC_{d}(S,W)\circ\DT(t)$ function $\vF'\equiv\vF|_\rho$ ($n$-bit output).
						
						If not all base-level CNF/DNF collapse to depth-$t$ decision trees, halt and output some constant function.
						
						\item For $j\in [i]$, $h_j'\equiv h_j$.
						
						\item $h'_{i+1}(y'_1,\ldots,y'_i):= h(y'_1,\ldots,y'_i)_{[m]}$.
						
						\item $h'(y'_1,\ldots,y'_{i+1}):= h(y'_1,\ldots,y'_i)_{\extInd(L(G(\D_R(y'_{i+1}))))}$.
						
						\item Finally, output $\tau'=(\vF',h'_1,\ldots,h'_{i+1},h')$.
					\end{enumerate}
					\medskip
				\end{minipage}}}
				\caption{Simulator, $\Sim$, for $(\E^\star,\D^\star)$}
				\label{fig:simulator}
			\end{figure}
			
			
			\begin{proof}[Proof of Lemma~\ref{thm:red}]
				Claim~\ref{cl:correctness} shows for any $x\in\zo^{k}$, $\Pr[\D^*(\E^*(x))=x]=1$. Now we prove for $\tau\in \leaky^{i,m,N}[\AC_d(S,W)\circ w\text{-}\AC_2(S')]$ defined by $(\vF,h_1,\ldots,h_i)$,  
				there exists a distribution $\Sim_{\tau}$ over $\tau'\in \leaky^{i+1,m,N}[\AC_{d}(S,W)\circ\DT(t)]$ such that for any $x$,  $\D^\star\circ\tau\circ\E^\star(x)$ is $\varepsilon$-close to $\tau'(x)$ when $\tau'$ is sampled from $\Sim_{\tau}$. $\Sim_{\tau}$ is defined in Figure\ref{fig:simulator}.
				
				
				Say that randomness $\zeta,U,r$ (where $r$ is the randomness for $\E_R$) is ``good for $\vF=(F_1,\cdots,F_N)$'' if 
				\begin{enumerate}
					\item the pseudorandom restriction $\rho$ formed by $\zeta,U,r$ as in both $S$ and $\E^\star$ collapses every DNF/CNF at the base of $\vF$ to an Decision Tree of height $t$, $\vF'\equiv\vF|_{\rho}$
					\item $(*)$ does not happen, i.e., there are enough stars in the pseudorandom restriction $\rho$.
				\end{enumerate}
				For convenience, we consider $\rho$ to be the resulting random restriction where there are exactly $|x|$ stars at the end, replacing any additional stars with draws from $\rho^{(2)}$.
				
				We will show that for any fixed, good $\zeta,U,r$ for $\vF$, $\D^\star\circ\tau\circ\E^\star(\cdot;\zeta,U,r)\equiv \tau'(\cdot)$, where $\tau'=S_{\tau}(\zeta,U,r)$.
					This follows from the fact that (1) and (2) hold: (1) $\vF'\equiv\vF|_\rho$ and (2) $\rho$ was used in both $\E^\star$ and $S_{\tau}$.
					It follows that for all $x$, $\vF'(x)=\vF|_\rho(x)=\vF(\vE(x;\zeta,R,r))$.
					Because $h_j'\equiv h_j$ for $j\in[i]$, it follows by induction that $y'_j=y_j$ (the output of each $h'_j$ and $h_j$ respectively, $j\in[i]$).
					Therefore, $h(y_1,\cdots,y_i)=h(y'_1,\cdots,y'_i)$.
					It follows that $\tilde{c}_{[m]}=y'_{i+1}$ and $L(G(\D_R(y'_{i+1})))=L(G(\tilde{\zeta}))$.  %\sgnote{step 5, No change; step 6, extract relevant tampering function indicies via leakage, and pull first $m$; step 7, given leakage and input $x$, again extract relevant tampering functions, then use $\vf$ to simulate the tampered seed and corresponding decoding locations.}
					Consequently, $h'(y'_1,\cdots,y'_{i+1})$ outputs that exact same indices that the decoding algorithm, $\D^\star$, will extract its output from. 
					Thus, $\tau'(x)=\D^\star\circ\tau\circ\E^\star(x;\zeta,R,r)$ for any $x$.  Because $\Sim$ and $\E^\star$ sample their randomness identically the distributions are identical, conditioned on the randomness being ``good.'' $\varepsilon$ is at most the probability that $\zeta,U,r$ are not ``good for \vF.''
				 
				Combining Claim~\ref{cl:error} and Lemma~\ref{lem:psl},
			    for any $\vF$, the probability that random $\zeta,U,r$ are not ``good for \vF'' is at most $\exp(-\Omega(\frac{\sigma}{\log(1/p)}))+NW(2^{w+t+1}(5pw)^t+\delta)$.  The desired conclusion follows.

							
\end{proof}

\iffalse
	We show will that the reduction $(\E^\star,\D^\star)$ allows us to trade depth for leakage.
	
	\begin{lemma}
		\label{thm:red}
		For $t=?,q=r(t,w,\log(1/\delta),\log n),p=?,n=?$, $d\in\bbN$,$S\in\bbN$
		$(\E_{q,p,n}^\star,\D_{q,p,n}^\star)$ is a ($\leaky^{k,m,N}[w-\AC_d(S)]\implies \leaky^{k+1,m,N}[\AC_{d-2}(S)\circ\DT(t)],\varepsilon$)-non-malleable reduction with rate ???,
		where $\varepsilon=?$.
		
		In particular, in the case that $d=2$,
		$(\E^\star,\D^\star)$ is a $(\leaky^{k,m,N}[w-\AC_d(S)]\implies\leaky^{k+1,m,N}[\DT(t)],\varepsilon)$-non-malleable reduction.
	\end{lemma}
	\mbnote{Will probably benefit from parametrizing size in a more tightly.}
	Combining the above with Proposition~\ref{prop:DT-DNF/CNF}.
	\begin{corollary}
		\label{cor:depth}
		For $t=?,q=r(t,w,\log(1/\delta),\log n),p=?,n=?$, $d\in\bbN$,$S\in\bbN$
		$(\E_{q,p,n}^\star,\D_{q,p,n}^\star)$ is a ($\leaky^{k,m,N}[w-\AC_d(S)]\implies \leaky^{k+1,m,N}[w-\AC_{d-1}(S')],\varepsilon$)-non-malleable reduction,
		where $\varepsilon=?$ and $S'=?$.
	\end{corollary}
	
	Additionally, if we consider $\vF\in\AC_d(S)$ to have an additional layer of fan-in 1 AND/OR gates, we get the following corollary.
	\begin{corollary}
		\label{cor:width}
		For $t=?,q=r(t,w,\log(1/\delta),\log n),p=?,n=?$, $d\in\bbN$,$S\in\bbN$
		$(\E_{q,p,n}^\star,\D_{q,p,n}^\star)$ is a ($\leaky^{k,m,N}[\AC_d(S)]\implies \leaky^{k+1,m,N}[w-\AC_{d}(S'),\varepsilon$)-non-malleable reduction,
		where $\varepsilon=?$ and $S'=S2^t$.
	\end{corollary}
	Combining the Corollary~\ref{cor:width} and many $d$ applications of Corollary~\ref{cor:depth} and the fact that $\AC_0\circ\DT(t)=\DT(t)\subseteq\Local^{2^t}$
	we get our main theorem:
	\begin{theorem}
		For any $d\in\mathbb{N}$,
		$(\underbrace{\E^\star\circ\cdots\circ\E^\star}_{\times d},\underbrace{\D^\star\circ\cdots\circ\D^\star}_{\times d})$
		is an $(\AC_d(S)\implies\leaky^{d,m,k}[\Local^{k^\delta}],d\varepsilon)$-non-malleable-reduction with rate $O(\log^{-O(d)}k)$, computable in time ???.
	\end{theorem}
	
	\begin{figure}[ht!]
		\fbox{\parbox{\textwidth}{

		\small \center
		\begin{minipage}{0.95\textwidth}
	given $\leaky^{k,m,N}[w-\AC_d(S)]$ tampering $\tau=(\vF,h_1,\ldots,h_k,h)$ output $\tau'=(\vF',h'_1,\ldots,h'_{k+1},h')$:
	\begin{enumerate}
	\item Draw (uniformly) random seed $\zeta\gets\{0,1\}^s$ 
	and (uniformly) random string $R\gets\{0,1\}^{n-m}$.
	
	\item Generate pseudorandom restriction, $\rho=(\rho^{(1)},\rho^{(2)})$:
	\begin{itemize}
		\item[] $\rho^{(1)} \gets L(G(\zeta))$. ($*$) If $\|L(G(\zeta))\|_0<k$ or $\extInd(L(G(\zeta)))_1\leq m$, set $\zeta=\zeta^{*}$. 
%			($*$) If the index of the $k$-th 1 in $L(G(\zeta))$ is $\leq n-m$
%			(or does not exist), 
%			use some fixed $\zeta^*$ such that
%			$\|L(G(\zeta^*))_{n-m+1,\ldots,n}\|_0\geq k$.
%			\mbnote{$k$ is overloaded}
%			(For $G$ from Lemma~\ref{lem:gen} such a $\zeta'$ can be found
%			via interpolation in time $O(q\log^2n)$.)
%		
		\item[] $\rho^{(2)} \gets \E_R(\zeta)\|R$
	\end{itemize}
	\item Apply (constructive) switching lemma with pseudorandom restriction to get $\AC_{d-1}\circ\DT(t)$ function $\vF'\equiv\vF|_\rho$ ($n$-bit output).
	
	If not all base-level CNF/DNF collapse to depth-$t$ decision trees, halt and output some constant function.
	
	\item For $i\in [k]$, $h_i'\equiv h_i$.
		\mbnote{No change.}
	\item $h'_{k+1}(y'_1,\ldots,y'_k):= h(y'_1,\ldots,y'_k)_{[m]}$.
	
		\mbnote{extract relevant tampering function indicies via leakage, and pull first $m$.}
	\item $h'(y'_1,\ldots,y'_{k+1}):= h(y'_1,\ldots,y'_k)_{\extInd(L(G(\D_R(y'_{k+1}))))}$.
	
	  \mbnote{given leakage and input $x$, again extract relevant tampering functions, then use $\vf$ to simulate the tampered seed and corresponding decoding locations.}
	\item Finally, output $\tau'=(\vF',h'_1,\ldots,h'_{k+1},h')$.
	\end{enumerate}
	\medskip
	\end{minipage}}}
	\caption{Simulator, $\Sim$, for $(\E^\star,\D^\star)$}
	\end{figure}
	
\begin{proof}[Proof of Lemma~\ref{thm:red}]
	Let $\tau\in \leaky^{k,m,N}[w-\AC_d(S)]$ defined by $(\vF,h_1,\ldots,h_k)$.
	
	Say that randomness $\zeta,R,r$ (where $r$ is the randomness for $\E_R$) is ``good for $\vF=(F_1,\cdots,F_N)$'' if 
	\begin{enumerate}
		\item the pseudorandom restriction $\rho$ formed by $\zeta,R,r$ as in both $S$ and $\E^\star$ collapses every DNF/CNF at the base of every $F_i$ to an Decision Tree of height $t$, $\vF'\equiv\vF|_{\rho}$
		\item $(*)$ does not happen, i.e., there are enough stars in the pseudorandom restriction $\rho$.
	\end{enumerate}
	For convenience, we consider $\rho$ to be the resulting random restriction where there are exactly $|x|$ stars at the end, replacing any additional stars with draws from $\rho^{(2)}$.
	
	For any $\vF$, the probability that random $\zeta,R,r$ are not ``good for \vF'' is at most $\exp(-q/2)+SN(2^{w+t+1}(5pw)^t+\delta)=\negl(n)$. This follows from Proposition~\ref{prop:red}, Lemma~\ref{lem:ind}, and Lemma~\ref{lem:psl}.
	
	Therefore it is suffices to show that for any fixed, good $\zeta,R,r$ for $\vF$, and we will show that $\D^\star\circ\tau\circ\E^\star(\cdot;\zeta,R,r)\equiv \tau'(\cdot)$, where $\tau'=S(\zeta,R,r)$.
	
	This follows from the fact that (1) and (2) hold: (1) $\vF'\equiv\vF|_\rho$ and (2) $\rho$ was used in both $\E^\star$ and $S$.
	It follows that for all $x$, $\vF'(x)=\vF|_\rho(x)=\vF(\vE(x;\zeta,R,r))$.
	Because $h_j'\equiv h_j$ for $j\in[k]$, it follows by induction that $y'_j=y_j$ (the output of each $h'_j$ and $h_j$ respectively, $j\in[k]$).
	Therefore, $h(y_1,\cdots,y_k)=h(y'_1,\cdots,y'_k)$.
	It follows that $\tilde{c}_[m]=y'_{k+1}$ and $L(G(\D_R(y'_{k+1})))=L(G(\tilde{\zeta}))$.
	Consequently, $h'(y'_1,\cdots,y'_{k+1})$ outputs that exact same indices that the decoding algorithm, $\D^\star$, will extract its output from. 
	Thus, $\tau'(x)=\D^\star\circ\tau\circ\E^\star(x;\zeta,R,r)$ for any $x$.
	
	Because $S$ and $\E^\star$ sample their randomness identically the distributions are identical, conditioned on the randomness being ``good.''
	
\end{proof}
\fi

==> preamble.tex <==


\RequirePackage{amsmath,amsthm,amsfonts,amssymb}
\RequirePackage{textcomp}

\usepackage{mathtools}
\usepackage{upgreek}
\usepackage{setspace}
\usepackage{multirow}
\usepackage{hyperref}
\usepackage{enumerate}


%\RequirePackage{fancybox}

\usepackage[dvipsnames]{xcolor}              % Need the color package
\usepackage{epsfig}
\usepackage{bm}
\usepackage[all]{xy}
\usepackage{tikz}
\usetikzlibrary{matrix}
\usepackage{fancybox}   

\usepackage{lipsum}
\usepackage[skins,breakable]{tcolorbox}

\RequirePackage{tcolorbox}

%\usepackage{fullpage}
\usepackage[margin=1in]{geometry}

\theoremstyle{plain}
%\theoremstyle{definition}


\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{Conjecture}{Conjecture}
\newtheorem{claim}{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem{property}{Property}
\newtheorem*{sketch}{Sketch}
\newtheorem*{note}{Note}
\newtheorem{example}{Example}
\newtheorem*{recall}{Recall}


\theoremstyle{definition}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}

%Shorthand
\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}

% \bbA, \bbB, ...
\def\ddef#1{\expandafter\def\csname bb#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \cA, \cB, ...
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \vA, \vB, ..., \va, \vb, ...
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz\ddefloop

% \valpha, \vbeta, ...,  \vGamma, \vDelta, ...,
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{\csname #1\endcsname}}}}
\ddefloop {alpha}{beta}{gamma}{delta}{epsilon}{varepsilon}{zeta}{eta}{theta}{vartheta}{iota}{kappa}{lambda}{mu}{nu}{xi}{pi}{varpi}{rho}{varrho}{sigma}{varsigma}{tau}{upsilon}{phi}{varphi}{chi}{psi}{omega}{Gamma}{Delta}{Theta}{Lambda}{Xi}{Pi}{Sigma}{varSigma}{Upsilon}{Phi}{Psi}{Omega}{ell}\ddefloop

\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\negl}{negl}

\newcommand{\E}{\mathrm{E}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\R}{\mathrm{R}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\Sim}{\mathrm{S}}
\newcommand{\Event}{\mathrm{EV}}
\newcommand{\eval}{\mathrm{Eval}}
\newcommand{\embed}{\mathrm{Embed}}
\newcommand{\extract}{\mathrm{Extract}}
\newcommand{\extInd}{\mathrm{ExtIndices}}

\newcommand{\cerr}{c_{\text{err}}}
\newcommand{\csec}{c_{\text{sec}}}
\newcommand{\crate}{c_{\text{rate}}}

\newcommand{\Local}{\mathrm{Local}}
\newcommand{\leaky}{\mathrm{LL}}

\newcommand{\ACZ}{\mathsf{AC^0}}
\newcommand{\AC}{\mathrm{AC}}
\newcommand{\NCZ}{\mathsf{NC^0}}
\newcommand{\dnf}{\mathrm{DNF}}
\newcommand{\DT}{\mathrm{DT}}
\newcommand{\p}{\mathsf{P}}
\newcommand{\nc}{\mathsf{NC}}

\newcommand{\zo}{\{0,1\}}

\iffalse
\newcommand{\mbnote}[1]{[{\footnotesize \color{DarkOrchid}{\bf marshall:} { {#1}}}]}
\newcommand{\sgnote}[1]{[{\footnotesize \color{blue}{\bf siyao:} { {#1}}}]}
\newcommand{\dnote}[1]{[{\footnotesize \color{green}{\bf dana:} { {#1}}}]}
\newcommand{\lynote}[1]{[{\footnotesize \color{red}{\bf li-yang:} { {#1}}}]}
\newcommand{\tmnote}[1]{[{\footnotesize \color{magenta}{\bf tal:} { {#1}}}]}
\fi

\iftrue
\newcommand{\mbnote}[1]{}
\newcommand{\sgnote}[1]{}
\newcommand{\dnote}[1]{}
\newcommand{\lynote}[1]{}
\newcommand{\tmnote}[1]{}
\fi

\newif\ifsubmission
\submissiontrue

\newcommand{\uhr}{\upharpoonright}

\newenvironment{myenum}
{ \begin{enumerate}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}     }
{ \end{enumerate}                  } 


%%%%%%%
%BDKM
%%%%%%%
\newcommand{\outloc}{\ell_\text{out}}
\newcommand{\inloc}{\ell_\text{in}}
\newcommand{\tdec}{t}
\newcommand{\tcheck}{t_\text{check}}
\newcommand{\cdec}{c_{\text{dec}}}
\newcommand{\cLerr}{c^L_\text{err}}
\newcommand{\cRerr}{c^R_\text{err}}
\newcommand{\cLsec}{c^L_\text{sec}}
\newcommand{\cRsec}{c^R_\text{sec}}
\newcommand{\cLrate}{c^L_\text{rate}}
\newcommand{\cRrate}{c^R_\text{rate}}
\newcommand{\nL}{n_L}
\newcommand{\nR}{n_R}
\newcommand{\nZ}{n_Z}
\newcommand{\PRGin}{s}
\newcommand{\tL}{t^L}
\newcommand{\tR}{t^R}
\newcommand{\sL}{s_L}
\newcommand{\sR}{S_R}
\newcommand{\affect}{A}


==> preliminaries-merged.tex <==
\section{Preliminaries}
\subsection{Basic Notation}
   For a positive integer $n$, let $[n]$ to denote $\{1,\dots,n\}$. For  $x=(x_1,\dots,x_n)\in\zo^n$, $\|x\|_0$ denotes the number of $1$'s in $x$.  For $i\leq j\in[n]$, we define $x_{i:j}:=(x_i,\dots,x_j)$. For a set $S\subseteq[n]$, $x_S$ denotes the projection of $x$ to $S$. For $S\in[n]^m$, $x_S:=(x_{S_1},\dots,x_{S_m})$. 
    For $x,y\in\zo^n$, if they disagree on at least $\varepsilon\cdot n$ indices, we say they are $\varepsilon$-far, otherwise, they are $\varepsilon$-close to each other.
   
   For a set $\Sigma$, we use $\Sigma^{\Sigma}$ to denote the set of all functions from $\Sigma$ to $\Sigma$. 
   Given a distribution $\mathcal{D}$, $z\leftarrow \mathcal{D}$ denotes sample $z$ according to $\mathcal{D}$. For two distributions $\mathcal{D}_1,\mathcal{D}_2$ over $\Sigma$, their statistical distance is defined as  $\Delta(\mathcal{D}_1,\mathcal{D}_2):=\frac{1}{2}\sum_{z\in\Sigma}|\mathcal{D}_1(z)-\mathcal{D}_2(z)å|$.
	 
	 We say $g(n)=\tilde{O}(f(n))$ if $g(n)=O(n^{\epsilon}f(n))$ for all $\epsilon>0$.
   
\subsection{Non-malleable Reductions and Codes}
	
		\begin{definition}[Coding Scheme] \cite{DPW10}
	  	A \emph{Coding scheme}, $(\E, \D)$, consists of a randomized
	 		encoding function $\E\colon \{0,1\}^k \mapsto \{0,1\}^n$ and a
	  	%randomized 
	  	decoding function $\D\colon \{0,1\}^n \mapsto
	  	\{0,1\}^k\cup\{\bot\}$ such that $\forall x \in \{0,1\}^k,
	  	\Pr[\D(\E(x))=x]=1$ (over randomness of $\E$). %(over randomness of $\E$ and $\D$).
		\end{definition}
		
Non-malleable codes were first defined in~\cite{DPW10}. Here we use a simpler, but equivalent, definition based on the following notion of non-malleable reduction by Aggarwal et al.~\cite{ADKO15}. 
		\begin{definition}[Non-Malleable Reduction] \cite{ADKO15} \label{def:red}
		  Let $\mathcal{F} \subset A^A$ and $\mathcal{G} \subset B^B$ be some classes of functions.
		  We say $\mathcal{F}$ \emph{reduces to} $\mathcal{G}$,
		  $(\mathcal{F} \Rightarrow \mathcal{G}, \varepsilon)$,
		  if there exists an efficient (randomized)  
		  encoding function $\E: B \to A$,  
		  and an efficient %(randomized) 
		  decoding function $\D: A \to B$,
		  such that
		  \begin{enumerate}[(a)]
		  \item $\forall x \in B, \Pr[\D(\E(x))=x]=1$ (over the
		  randomness of $\E$). %(over the randomness of $\E, \D$).
		  \item $\forall f \in \mathcal{F},\exists G$ s.t. $ \forall x \in B$,
		    $\Delta(\D(f(\E(x)));G(x))\leq \varepsilon$,
		    where $G$ is a distribution over $\mathcal{G}$ and $G(x)$ denotes the distribution $g(x)$, where $g \leftarrow G$.
		  \end{enumerate}
		  If the above holds, then $(\E,\D)$ is an \emph{$(\mathcal{F},\mathcal{G},\varepsilon)$-non-malleable reduction}.
		\end{definition}

		\begin{definition}[Non-Malleable Code] \cite{ADKO15}
		  Let $\textsc{NM}_k$ denote the set of \emph{trivial manipulation functions} on $k$-bit strings,
		  consisting of the identity function $\text{id}(x)=x$ and all constant functions $f_c(x)=c$, where $c \in \{0,1\}^k$.

		  A coding scheme $(\E,\D)$ defines an \emph{$(\mathcal{F}_{n(k)},k,\varepsilon)$-non-malleable code},
		  if it defines an $(\mathcal{F}_{n(k)},\textsc{NM}_k,\varepsilon)$-non-malleable reduction.
			
			Moreover, the rate of such a code is taken to be $k/n(k)$.
		\end{definition}
	%	\mbnote{I modified what we had here previously...}
		
		  The following useful theorem allows us to compose non-malleable reductions.
		\begin{theorem} [Composition] \cite{ADKO15}  \label{thm:composition}
		  If $(\mathcal{F} \Rightarrow \mathcal{G}, \varepsilon_1)$
		  and $(\mathcal{G} \Rightarrow \mathcal{H}, \varepsilon_2)$,
		  then $(\mathcal{F} \Rightarrow \mathcal{H}, \varepsilon_1 + \varepsilon_2)$.
		\end{theorem}
		
		\subsection{Tampering Function Families}
		\subsubsection{Split-State and Local Functions}
			
			\begin{definition}[Split-State Model] \cite{DPW10}
				The \emph{split-state model}, $\textsc{SS}_k$, denotes the set of all functions:
				\[\{f=(f_1,f_2):\ f(x)=(f_1(x_{1:k})\in\{0,1\}^k,f_2(x_{k+1:2k})\in\{0,1\}^{k}) \mbox{ for } x\in\{0,1\}^{2k}\}.\]
			\end{definition}
			
			\begin{theorem}[Split-State NMC]\cite{Li17}
				\label{thm:ss-nmc}
				For any $n\in\mathbb{N}$,
				there exists an explicit, efficient non-malleable code in the 2-split-state model with rate $k/n=\Omega(1/ \log n)$ and error $2^{-\Omega(k)}$
			\end{theorem}
			%k/n = 1/log n ==> k = n/\log n
			
			\begin{definition}[Local Functions]
				Let  $f: \{0,1\}^n \to \{0,1\}^m$ be a function. We say output $j$ of $f$ \emph{depends} on input $i$  %or input $i$  \emph{affects} output $j$ of $f$ 
				if there exists $x,x'\in\{0,1\}^n$ that differ only in the $i$th coordinate such that $f(x)_j\neq f(x')_j$. We say $f$ is $\ell$-local or in the class $\Local^{\ell}$, if every output bit $f_j$ depends on at most $\ell$ input bits. 
			\end{definition}
			
			
			
		
		\subsubsection{Low Depth Circuits and Decision Trees}
		A Boolean circuit with $n$ input bits is a directed acyclic graph in which every node (also called gate) is either an input node of in-degree $0$ labeled by one of the $n$ input bits, an AND gate, an OR gate, or a NOT gate.  One of these gates is designated as the output gate.  The {\em size} of a circuit is its numebr of gates and the {\em depth} of a circuit is the length of its longest path from an input gate to the output gate. 
		
		
		 Throughout the paper, we assume that NOT gates are only applied at in input level. 
		 Moreover, we assume that circuits are {\em layered} so that a gate at layer $i$ takes inputs only from gates at layer $i-1$ and the gate at layer $1$ takse as inputs only the inputs of the circuit, and circuits are {\em alternating}, namely each layer contains either only OR gates or only AND gates and  Layers with AND gates and Layers with OR gates alternate.  This is without loss of generality because a circuit of size $S$ and depth $d$ can be transformed into a circuit of size at most $dS$ and depth $d$ which satisfies those conditions and computes the same function.
		
		 Let $\AC_d(S)$ denote alternating depth $d$ circuits of size at most $S$ with unbounded fan-in. 
		 %For clarity, we take $\AC_d(S,W)$ to denote $\AC_d(S)$ with width at most $W$. Although at small depth, width and size are essentially equivalent: $W\leq S\leq dW$.
		 Let $w$-$\AC_d(S)$ denote alternating depth $d$ circuits of size at most $S$ with fan-in at most $w$ at the the first level and unbounded fan-in elsewhere.   For depth $2$ circuits, a DNF is an OR of ANDs (terms) and a CNF is an AND or ORs (clauses). The {\em width} of a DNF (respectively, CNF) is the maximum number of variables that occur in any of its terms (respectively, clauses).  We use $w$-DNF to denote the set of DNFs with width at most $w$.
		 
		 
		 A decision tree with $n$ input bits is a binary tree whose internal nodes have labels from $x_1,\dots,x_n$ and whose leaves have labels from $\zo$. If a node has label $x_i$ then the test performed at that node is to examine the $i$-th bit of the input. If the result is $0$, one descends into the left subtree , whereas if the result is $1$, one descends into the right subtree. The label of the leaf so reached is the output value on that particular input.  The {\em depth} of a decision tree is the number of edges in a longest path from the root to a leaf. Let $\DT(t)$ denote  decision trees with depth at most $t$. 
		 
		 Here are some useful facts relating decision trees and depth $2$ circuits and local functions.  A decision tree of depth $t$ can be computed by a $t$-DNF (respectively $t$-CNF) by, for each path associated with a leaf with value $1$ (respectively value $0$), forming a corresponding clause (respectively term) using variables on the path. A boolean function $f$ computed by any depth $t$ decision tree is $2^t$-local because $f$ only depends on variables labeled on the tree and there are at most $2^t$ variables are labeled on a binary tree of depth $t$.
		 
		 $\AC_d(S)\circ\DT(t)$ denotes alternating (unbounded fan-in) circuits of depth $d$, size $S$ that take the output of depth $t$ decision trees as input.
		(Note may contain up to $S$ decision trees.)
		Similarly it is helpful to decompose an alternating circuit (from $w$-$\AC_d$) into a base layer of CNFs or DNFs and the rest of the circuit, $\AC_{d-2}(S)\circ w$-$\AC_2(S')$. (Again, the base may contain up to $S$ CNFs/DNFs of size $S'$.)  
		
		
		For a set of boolean circuits $\cC$ (respectively decision trees), we say that a boolean function $f$ is in $\cC$, if there exists a $C\in\cC$ which agrees with $f$ on every input. We say that a multiple output function $f=(f_1,\dots,f_m)$ is in $\cC$ if $f_i\in \cC$ for any $i\in[m]$.
		

\subsubsection{Leaky Function Families}
		Given an arbitrary class of tampering functions, we consider a variant of the class of tampering functions which may depend in some limited way on limited leakage from the underlying code word. 
		
		
		\begin{definition} [Leaky Function Families]
		Let $\leaky^{i,m,N}[\cC]$ denote tampering functions generated via the following game:
		\begin{enumerate}
			\item The adversary first commits to $N$ functions from a class $\cC$,
			$F_1,\ldots,F_N = \vF$.
			
			(Note: $F_j:\zo^N\to\zo$ for all $j\in[N]$.) 
			
			\item The adversary then has $i$-adaptive rounds of leakage. In each round $j\in[i]$,
			\begin{itemize}
				\item the adversary selects $s$ indices from $[N]$, denoted $S_j$,
				\item the adversary  receives $\vF(x)_{S_j}$.
				\end{itemize}
				
				Formally, we take $h_j:\zo^{m(j-1)}\to[N]^m$ to be the selection function such that    \[h_j(F(X)_{S_1},\ldots,F(X)_{S_{j-1}})=S_{j}.\]
				Let $h_1$ be the constant function that outputs $S_1$.
				
			\item Finally, selects a sequence of $n$ functions $(F_{t_1},\ldots,F_{t_n})$ ($T=\{t_1,\ldots,t_n\}\subseteq[N]$ such that $t_1<t_2<\cdots<t_n$) to tamper with.
			
				Formally, we take $h:\zo^{mi}\to [N]^n$ such that
				$h(F(X)_{S_1},\ldots,F(X)_{S_i})=T$.
		\end{enumerate}
		Thus, any $\tau\in\leaky^{i,m,N}[\cC]$ can be described via $(\vF,h_1,\cdots,h_i,h)$. In particular, we take $\tau = \eval(\vF,h_1,\cdots,h_i,h)$ to denote the function whose output given input $X$ is $T(X)$, where $T$ is, in turn, outputted by the above game given input $X$ and adversarial strategy $(\vF,h_1,\cdots,h_i,h)$.
		\end{definition}
		
\subsection{Pseudorandom Ingredients}
\subsubsection{A Binary Reconstructible Probabilistic Encoding Scheme}
Reconstructable Probabilistic Encoding (RPE) schemes were first introduced by Choi et al.~\cite{CDMW08, CDMW16}. Informally, RPE is a combination of error correcting code and secret sharing, in particular, it is an error correcting code with an additional secrecy property and reconstruction property.
\begin{definition}[Binary Reconstructable Probabilistic Encoding] 
	\cite{CDMW08,CDMW16}
	We say a triple $(\E, \D, \R)$ is a {\sf binary reconstructable probabilistic
		encoding scheme} with parameters $(k, n, \cerr, \csec)$, where
	$k, n \in \bbN$, $0 \leq \cerr,\csec < 1$, if it
	satisfies the following properties: 
	
	\begin{enumerate}
		\item \textbf{Error correction.} 
		$\E\colon \zo^k \rightarrow \zo^n$ is an efficient probabilistic
		procedure, which maps a message $x \in \zo^k$ to a distribution over
		$\zo^n$. If we let $\cC$ denote the support of $\E$, any two
		strings in $\cC$ are $2\cerr$-far.
		Moreover, $\D$ is an efficient procedure that
		given any $w' \in \zo^n$ that is $\epsilon$-close to some string $w$ in
		$\cC$ for any $\epsilon \leq \cerr$, outputs $w$ along with a consistent $x$.
		\item \textbf{Secrecy of partial views.} 
		For all $x \in \zo^k$ and any non-empty set $S \subset [n]$ of size $\leq \lfloor\csec\cdot n\rfloor$, $\E(x)_S$ is
		identically distributed to the uniform distribution over $\zo^{|S|}$.  
		
		
		\item \textbf{Reconstruction from partial views.} 
		$\R$ is an efficient procedure that given any set $S \subset [n]$ of size $\leq \lfloor\csec\cdot n\rfloor$,
		any $\hat{c} \in \zo^n$, and any $x \in \zo^k$, samples
		from the distribution $\E(x)$ with the constraint  $\E(x)_S={\hat{c}}_S$.  
	\end{enumerate}
\end{definition}

\begin{lemma} \cite{CDMW08,CDMW16}%thm 2.1
	\label{lem:rpe}
	For any $k \in \bbN$,
	there exist constants $0<\crate,\cerr,\csec<1$ such that
	there is a binary RPE scheme with parameters
	$(k, \crate k, \cerr, \csec)$.
\end{lemma}


To achieve longer encoding lengths $n$, with the same $\cerr,\csec$  parameters, one can simply pad the message to an appropriate length.  

RPE was been used in Ball et al.\cite{BDKM16} for building non-malleable reductions from local functions to split state functions.  However, for all reductions in our paper, error correction property is not necessary (RPE $\cerr=0$ is adequate). In addition, we observe that RPEs with parameters $(k,n,0,\csec)$ are implied by any linear error correcting code with parameters $(k,n,d)$ where $k$ is the message length, $n$ is the codeword length, $d:=\csec\cdot n+1$ is the minimal distance. 

\begin{lemma}\label{lm:wRPE}
	Suppose there exists a binary linear error correcting code with parameters $(k,n,d)$, then there is a binary RPE scheme with parameters $(k,n,0,(d-1)/n)$.
\end{lemma}


\begin{proof}
	For a linear error correcting code with $(k,n,d)$,  let $A$ denote its encoding  matrix, $H$ denote its parity check matrix. Let $B$ be a matrix so that $BA=I$ where $I$ is the $k\times k$ identity matrix (such $B$ exists because $A$ has  rank $k$ and can be found efficiently). By property of parity check matrix, $HA=\bold{0}$ and $Hs\neq 0$ for any $0< ||s||_0<d$  where $\bold{0}$ is the $(n-k)\times k$ all $0$ matrix.
	
	We define $(\E,\D,\R)$ as follows: for $x\in\zo^k$ and randomness $r\in\zo^{n-k}$, $\E(x;r):=B^Tx+H^Tr$, for $c\in\zo^{n}$; $\D(c):=A^Tc$; given $S \subset [n]$ of size $\leq d-1$ , $\hat{c} \in \zo^n$,  $x \in \zo^k$, $\R$ samples $r$ uniformly from the set of solutions to $(H^Tr)_S=(\hat{c}-B^Tx)_S$ then outputs $\E(x;r)$. 
	
	$(\E,\D)$ is an encoding scheme because  $\D\circ\E =A^TB^T=I^T=I$.  For secrecy property, note that for any non-empty $S\subseteq[n]$ of size at most $d-1$, $(Hr)_S$ is distributed uniformly over $\zo^{|S|}$, because for any $a\in\zo^{|S|}$, \[\Pr_{r}[(H^Tr)_S=a]=\E[\Pi_{i\in S}\frac{1+(-1)^{(H^Tr)_i+a_i}}{2}]=2^{-|S|}\sum_{S'\subseteq S} \E[\Pi_{i\in S'}(-1)^{(H^Tr)_i+a_i}]=2^{-|S|},\]
	where the last equality is because the only surviving term is $S'=\emptyset$ and for other $S'$, $\sum_{i\in S'}H^T_i\neq 0$ so $\E[\Pi_{i\in S'}(-1)^{(H^Tr)_i}]=0$.
	It implies $\E(x)_S$ is also distributed uniformly over $\zo^{S}$. By definition, $R$ satisfies reconstruction property.  Hence $(\E,\D,\R)$ is a binary RPE with parameters $(k,n,0,(d-1)/n)$.
	
\end{proof}





\subsubsection{A Simple $\sigma$-wise Independent Generator}

\begin{definition} [Bounded-independent Generator] We say a distribution $\mathcal{D}$ over $\zo^n$ is {\em $\sigma$-wise independent} if for any $S\subseteq [n]$ of size at most $\sigma$, $\mathcal{D}_S$ distributes identically to the uniform distribution over $\zo^{|S|}$. We say function $G\colon\zo^s\rightarrow\zo^n$ is a $\sigma$-wise independent generator if $G(\zeta)$ is $\sigma$-wise independent where $\zeta$ is uniformly distributed over $\zo^s$.	
\end{definition}

The simple Carter-Wegman hashing construction based on random polynomials suffices for our purposes.
\begin{lemma}
	\label{lem:gen}
	\cite{CW81}
	There exists an (explicit) $\sigma$-wise independent generator:
	$G:\zo^{(\sigma+1)\log n}\to\zo^{n}$, computable in time $\tilde{O}(\sigma n)$.
	
	Moreover, $G:\zo^{(\sigma+1)m}\to\zo^n$ can be constructed such that for an subset $S\subseteq[n]$ of size $\sigma$, $G(\zeta)_S \equiv X_1,\ldots,X_\sigma$ (for uniformly chosen $\zeta$) where (1) $X_i$'s are independent Bernoullis with $\Pr[X_i=1]=q/d$ for $q\in\{0,\ldots,d\}$, and (2) $m=\max\{\log n,\log d\}$.
\end{lemma}

Let $G_{\sigma,p}$ denote a $\sigma$-wise independent Carter-Wegman generator with bias $p$, and $G_{\sigma}$ such a generator with $p=1/2$

The following useful theorem gives Chernoff-type concentration bounds for $\sigma$-wise independent distributions. %(not to mention the previous section).
\begin{theorem}[\cite{SSS95}]
	\label{thm:pr-chernoff}
	If $X$ is a sum of $\sigma$-wise independent random indicator variables with $\mu=\bbE[X]$, then $\forall\epsilon: 0<\varepsilon\leq1,\sigma\leq\varepsilon^2\mu e^{-1/3}$, 
	$\Pr[|X-\mu|>\varepsilon\mu] < \exp(-\lfloor \sigma/2 \rfloor)$.
\end{theorem}	
\iffalse
\subsubsection{The Pseudorandom Switching Lemma of Trevisan and Xue}
\begin{definition}
	\label{def:enc-prr}
	Fix $p\in(0,1)$.
	A string $s\in\zo^{n\times \log(1/p)}$ encodes a subset 
	$L(s)\subseteq[n]$ as follows:
	for each $i\in[n]$,
	\[ i\in L(s) \iff s_{i,1}=\cdots=s_{i,\log(1/p)}=1.\]
\end{definition}

\begin{definition}
	\label{def:prr}
	Let $\cD$ be a distribution over $\zo^{n\log(1/p)}\times\zo^n$.
	This distribution defines a distribution $\cR(\cD)$ over restrictions $\{0,1,*\}^n$,
	where a draw $\rho\gets\cR(\cD)$ is sampled as follows:
	\begin{enumerate}
		\item Sample $(s,y)\gets \cR(\cD)$,
		where $s\in\zo^{n\log(1/p)},y\in\zo^n$.
		\item Output $\rho$ where
		\begin{align*}
			\rho_i := \left\{
			\begin{array}{rl}
				y_i &\mbox{if } i\notin L(s)\\
				* &\mbox{otherwise}
			\end{array}
			\right.
		\end{align*}
	\end{enumerate}
\end{definition}

\begin{theorem}[Polylogarithmic independence fools CNF formulas~\cite{Baz09,Raz09}] 
\label{thm:bazzi} 
The class of $M$-clause CNF formulas is $\epsilon$-fooled by $O((\log(M/\epsilon))^2)$-wise independence. 
\end{theorem}

\begin{theorem}[A Pseudorandom version of H{\aa}stad's switching lemma~\cite{Hastad86,TX13}] 
\label{thm:TX-SL} 
Fix $p,\delta \in (0,1)$ and $w, S, t\in \bbN$. There exists a value $r \in \bbN$, 
\[ r = \poly(t,w,\log(S), \log(1/\delta), \log(1/p)),\footnote{The exponent of this polynomial is a fixed absolute constant independent of all other parameters.}  \]
 such that the following holds.  Let $\cD$ be any $r$-wise independent distribution over $\zo^{n\times \log(1/p)} \times \zo^n$ \footnote{Recall that an $r$-wise independent distribution over $\zo^m$ can be generated with seed length $O(r\log m)$. In this case, $m = n\times \log(1/p) + n$ so this is $O(r \log (n \log(1/p)))$.} .  If $F : \zo^n \to \zo$ is a size-$S$ depth-$2$ circuit with bottom fan-in $w$, then 
 \[ \Pr\big[\, \DT(F \uhr \vrho) \ge t \, \big] \le 2^{w+t+1} (5pw)^t + \delta, \]
 where the probability is taken with respect to a pseudorandom restriction $\vrho\leftarrow\cR(\cD)$.  
\end{theorem} 

\begin{proof} 
By Lemma 7 of~\cite{TX13}, any distribution $\cD'$ over $\zo^{n\times \log(1/p)} \times \zo^n$ that $\epsilon$-fools the class of all 
$(S\cdot 2^{w(\log(1/p)+1)})$-clause CNFs satisfies
\[ \Pr\big[\, \DT(F \uhr \vrho) \ge t \, \big] \le 2^{w+t+1} (5pw)^t + \epsilon\cdot 2^{(t+1)(2w+\log S)},  \]
where the probability is taken with respect to a pseudorandom restriction $\vrho\leftarrow\cR(\cD')$.  By Theorem~\ref{thm:bazzi}, the class of $M := (S\cdot 2^{w(\log(1/p)+1)})$-clause CNF formulas is 
\[ \epsilon := \delta \cdot 2^{-(t+1)(2w+\log S)}\] 
fooled by $r$-wise independence where 
\[ r= O((\log(M/\epsilon))^2) =   \poly(t,w,\log(S), \log(1/\delta), \log(1/p)), \]
and the proof is complete.  
\end{proof} 

Taking a union bound we get the following corollary.
\begin{corollary}
	\label{lem:psl}
Fix $p,\delta \in (0,1)$ and $w, S, t \in \bbN$. There exists a value $r \in \bbN$, 
\[ r = \poly(t,w,\log(S), \log(1/\delta), \log(1/p)),   \]
 such that the following holds.  Let $\cD$ be any $r$-wise independent distribution over $\zo^{n\times \log(1/p)} \times \zo^n$. 
 Let $F_1,\ldots,F_M$ be $M$ many size-$S$ depth-$2$ circuits with bottom fan-in $w$.  Then 
\begin{equation} \Pr_{\vrho\leftarrow\cR_p}\Big[ \exists\, j \in [M] \text{~such that~} \DT(F_j \uhr \vrho) \ge t \,\Big] \le M\cdot \left(2^{w+t+1} (5pw)^{t} + \delta\right).  \label{eq:pseudorandom-failure} 
\end{equation} 
 \end{corollary} 
\fi
\iffalse
The following is a simple corollary of the pseudorandom switching lemma in~\cite{TX13}.

\begin{lemma}[Pseudorandom Switching Lemma]
	\label{lem:psl}
	\cite{TX13}
	
	Fix $(p,\delta)\in(0,1)$ and $w,S,t\in\bbN$.
	Then, there exists a value $r\in\bbN$,
	\[r=\poly(t, w,\log(S),\log(1/\delta),\log(1/p))\footnote{The exponent of this polynomial is a fixed absolute constant independent of all other paramemters.}\]
	such that the following holds.
	
	Let $\cD$ be any $r$-wise independent distribution over $\zo^{n\log(1/p)}\times\zo^n$.
	Let $F=F_1,\ldots,F_M$ where $F_1,\dots,F_M$ are size-$S$ depth-$2$ circuits with bottom fan-in $w$,
	then
	\[\Pr_{\rho\gets\cR(\cD)}\left[F_\rho\text{ is not in }\DT(t)\right]
	\leq M\left(2^{w+t+1}(5pw)^{t}+ \delta\right).\]
\end{lemma}
\fi

\subsection{Helpful Functions.}

Lastly, we define some convient functions. For a random restriction  $\rho=(\rho^{(1)},\rho^{(2)})\in\{0,1\}^{n}\times\zo^{n}$, $\extInd(\rho^{(1)}):=(i_1,\ldots,i_k)\in [n+1]^k$ are the last $k$ indices of 1s in $\rho^{(1)}$ where $i_1\leq i_2\dots\leq i_k$ and $i_j=n+1$ for $j\in[k]$ if such index doesn't exist ($k$ should be obvious from context unless otherwise noted).  

We define a pair of functions for embedding and extracting a string $x$  according to a random restriction, $\rho$. Let $\embed:\zo^{k+2n}\to\zo^n$, 
such that for $\rho=(\rho^{(1)},\rho^{(2)})\in\{0,1\}^{n}\times\zo^{n}$ and $x\in\{0,1\}^k$, and $i\in[n]$,
	
	%\\ if $i=\extInd(\rho^{(1)})_j$ for some $j\in[k]$ then $\embed(x,\rho)_i:= x_j$ otherwise $\embed(x,\rho)_i:= x_j$.
	\begin{equation*}
		\embed(x,\rho)_i = 
		\left\{\begin{array}{rl}
			x_j & \mbox{if } \exists j\in[k]: i=\extInd(\rho^{(1)})_j \\
			\rho_i^{(2)} & \mbox{otherwise}\\
		\end{array}\right.
	\end{equation*}
	And, let $\extract:\zo^{2n}\to\zo^k\times\{\bot\}$ be such that if $c\in\zo^n,\rho^{(1)}\in\{0,1\}^n$, and $\|\rho^{(1)}\|_0\geq k$,
	then $\extract(c,\rho^{(1)})=c_{\extInd(\rho^{(1)})}$.
	Otherwise, $\extract(c,\rho^{(1)})=\bot$.

Note that, for any $\rho$ such that  $\|\rho^{(1)}\|_0\geq k$, $\extract(\embed(x,(\rho^{(1)},\rho^{(2)})),\rho^{(1)})=x$.


==> preliminaries.tex <==

\iffalse
\subsection{Models of Computation.}
\mbnote{expand}

$\AC_d(S)$ denotes alternating depth $d$ circuits of size at most $S$ with unbounded fan-in.
$w$-$\AC_d(S)$ denotes alternating depth $d$ circuits of size at most $S$ with fan-in at most $w$ at the the first level and unbounded fan-in elsewhere. 	$\DT(t)$ denotes decision trees of depth at most $t$.

$\AC_d(S)\circ\DT(t)$ denotes alternating (unbounded fan-in) circuits of depth $d$, size $S$ that take the output of depth $t$ decision trees as input.
(Note may contain up to $S$ decision trees.)
\fi

   \subsection{Basic Notation}
   For a positive integer $n$, let $[n]$ to denote $\{1,\dots,n\}$. For  $x=(x_1,\dots,x_n)\in\zo^n$, $\|x\|_0$ denotes the number of $1$'s in $x$.  For $i\leq j\in[n]$, we define $x_{i:j}:=(x_i,\dots,x_j)$. For a set $S\subseteq[n]$, $x_S$ denotes the projection of $x$ to $S$. For $S\in[n]^m$, $x_S:=(x_{S_1},\dots,x_{S_m})$. 
    For $x,y\in\zo^n$, if they disagree on at least $\varepsilon\cdot n$ indices, we say they are $\varepsilon$-far, otherwise, they are $\varepsilon$-close to each other.
   
   For a set $\Sigma$, we use $\Sigma^{\Sigma}$ to denote the set of all functions from $\Sigma$ to $\Sigma$. 
   Given a distribution $\mathcal{D}$, $z\leftarrow \mathcal{D}$ denotes sample $z$ according to $\mathcal{D}$. For two distributions $\mathcal{D}_1,\mathcal{D}_2$ over $\Sigma$, their statistical distance is defined as  $\Delta(\mathcal{D}_1,\mathcal{D}_2):=\frac{1}{2}\sum_{z\in\Sigma}|\mathcal{D}_1(z)-\mathcal{D}_2(z)å|$.
	 
	 We say $g(n)=\tilde{O}(f(n))$ if $g(n)=O(n^{\epsilon}f(n))$ for all $\epsilon>0$.
   
	
	\subsection{Non-malleable Reductions and Codes}
	
		\begin{definition}[Coding Scheme] \cite{DPW10}
	  	A \emph{Coding scheme}, $(\E, \D)$, consists of a randomized
	 		encoding function $\E\colon \{0,1\}^k \mapsto \{0,1\}^n$ and a
	  	%randomized 
	  	decoding function $\D\colon \{0,1\}^n \mapsto
	  	\{0,1\}^k\cup\{\bot\}$ such that $\forall x \in \{0,1\}^k,
	  	\Pr[\D(\E(x))=x]=1$ (over randomness of $\E$). %(over randomness of $\E$ and $\D$).
		\end{definition}
	%	\mbnote{here, unlike in~\cite{DPW10}, we allow randomized decoding.}	\sgnote{I changed it back to deterministic decoding because we don't need randomized decoding.}
\iffalse		
			\subsubsection{Reconstructible}
			\begin{definition}[Binary Reconstructable Probabilistic Encoding] 
				\cite{CDMW08,CDMW16}
				We say a triple $(\E, \D, \R)$ is a {\sf binary reconstructable probabilistic
					encoding scheme} with parameters $(k, n, \cerr, \csec)$, where
				$k, n \in \bbN$, $0 < \cerr,\csec < 1$, if it
				satisfies the following properties: 
				
				\begin{enumerate}
					\item \textbf{Error correction.} 
					$\E\colon \zo^k \rightarrow \zo^n$ is an efficient probabilistic
					procedure, which maps a message $x \in \zo^k$ to a distribution over
					$\zo^n$. If we let $\cC$ denote the support of $\E$, any two
					strings in $\cC$ are $2\cerr$-far.
					Moreover, $\D$ is an efficient procedure that
					given any $w' \in \zo^n$ that is $(1-\epsilon)$-close to some string $w$ in
					$\cC$ for any $\epsilon \leq \cerr$, outputs $w$ along with a consistent $m$.
					\item \textbf{Secrecy of partial views.} 
					For all $m \in \zo^k$ and all sets $S \subset [n]$ of size $\leq \lfloor\csec\cdot n\rfloor$, the
					projection of $\E(x)$ onto the coordinates in $S$, as denoted by $\E(x)|_S$, is
					identically distributed to the uniform distribution over $\zo^{\lfloor\csec n\rfloor}$.
					
					\item \textbf{Reconstruction from partial views.} 
					$\R$ is an efficient procedure that given any set $S \subset [n]$ of size $\leq \lfloor\csec\cdot n\rfloor$,
					any $\hat{c} \in \zo^n$, and any $x \in \zo^k$, samples
					from the distribution $\E(x)$ with the constraint $ \forall i \in S, {\E(x)}_i = {\hat{c}}_i$.  
				\end{enumerate}
			\end{definition}
			
		
		\subsubsection{Non-malleable.}
	
		
		\begin{definition}[Non-Malleable Code] \cite{ADKO15} 			%\cite{ITCS:DziPieWic10}
		  Let $\mathcal{F}$ denote a family of tampering functions.
		  Let $\E\colon B\to A$, $\D\colon A\to B$ be a coding scheme.
		%
		  For all $f\in\mathcal{F}$ and all $x\in B$ define:
		  \[\text{Tamper}^f_x:=\{c\leftarrow\E(x);\tilde{c}\leftarrow f(c); \tilde{x}\leftarrow D(\tilde{c}); \mbox{ output: }\tilde{x}\}.\]
		%
		  Then, $(\E,\D)$ is an $\varepsilon$-non-malleable code with respect to $\mathcal{F}$, if for any $f\in\mathcal{F}$, there exists a distribution
		  $D_f$ over $\{0,1\}^k\cup\{\bot,\mbox{same}\}$ such that $\forall x \in B$, the statistical distance between
		  \[\text{Sim}_x^f:=\{\tilde{x}\leftarrow D_f; \mbox{ output: } x \mbox{ if } \tilde{x}=\mbox{same}\ \&\ \tilde{x},\mbox{ otherwise}\},\]
		  and $\text{Tamper}^f_x$ is at most $\varepsilon$.
		\end{definition}
\fi

Non-malleable codes were first defined in~\cite{DPW10}. Here we use the simpler alternative equivalent definition based on the following notion of non-malleable reduction by Aggarwal et al.~\cite{ADKO15}. 
		\begin{definition}[Non-Malleable Reduction] \cite{ADKO15} \label{def:red}
		  Let $\mathcal{F} \subset A^A$ and $\mathcal{G} \subset B^B$ be some classes of functions.
		  We say $\mathcal{F}$ \emph{reduces to} $\mathcal{G}$,
		  $(\mathcal{F} \Rightarrow \mathcal{G}, \varepsilon)$,
		  if there exists an efficient (randomized)  
		  encoding function $\E: B \to A$,  
		  and an efficient %(randomized) 
		  decoding function $\D: A \to B$,
		  such that
		  \begin{enumerate}[(a)]
		  \item $\forall x \in B, \Pr[\D(\E(x))=x]=1$ (over the
		  randomness of $\E$). %(over the randomness of $\E, \D$).
		  \item $\forall f \in \mathcal{F},\exists G$ s.t. $ \forall x \in B$,
		    $\Delta(\D(f(\E(x)));G(x))\leq \varepsilon$,
		    where $G$ is a distribution over $\mathcal{G}$ and $G(x)$ denotes the distribution $g(x)$, where $g \leftarrow G$.
		  \end{enumerate}
		  If the above holds, then $(\E,\D)$ is an \emph{$(\mathcal{F},\mathcal{G},\varepsilon)$-non-malleable reduction}.
		\end{definition}

		\begin{definition}[Non-Malleable Code] \cite{ADKO15}
		  Let $\textsc{NM}_k$ denote the set of \emph{trivial manipulation functions} on $k$-bit strings,
		  consisting of the identity function $\text{id}(x)=x$ and all constant functions $f_c(x)=c$, where $c \in \{0,1\}^k$.

		  A coding scheme $(\E,\D)$ defines an \emph{$(\mathcal{F},k,\varepsilon)$-non-malleable code},
		  if it defines an $(\mathcal{F},\textsc{NM}_k,\varepsilon)$-non-malleable reduction.
		\end{definition}
		
		  The following useful theorem allows us to compose non-malleable reductions.
		\begin{theorem} [Composition] \cite{ADKO15}  \label{thm:composition}
		  If $(\mathcal{F} \Rightarrow \mathcal{G}, \varepsilon_1)$
		  and $(\mathcal{G} \Rightarrow \mathcal{H}, \varepsilon_2)$,
		  then $(\mathcal{F} \Rightarrow \mathcal{H}, \varepsilon_1 + \varepsilon_2)$.
		\end{theorem}
		
		\subsection{Tampering Function Families}
		\subsubsection{Split-State and Local Functions}
			
			\begin{definition}[Split-State Model] \cite{DPW10}
				The \emph{split-state model}, $\textsc{SS}_k$, denotes the set of all functions:
				\[\{f=(f_1,f_2):\ f(x)=(f_1(x_{1:k})\in\{0,1\}^k,f_2(x_{k+1:2k})\in\{0,1\}^{k}) \mbox{ for } x\in\{0,1\}^{2k}\}.\]
			\end{definition}
			
			\begin{theorem}[Split-State NMC\cite{Li17}]
				\label{thm:ss-nmc}
				For any $n\in\mathbb{N}$,
				there exists an explicit, efficient non-malleable code in the 2-split-state model with rate $k/n=\Omega(1/ \log n)$ and error $2^{-\Omega(k)}$
			\end{theorem}
			%k/n = 1/log n ==> k = n/\log n
			
			\begin{definition}[Local Functions]
				Let  $f: \{0,1\}^n \to \{0,1\}^m$ be a function. We say output $j$ of $f$ \emph{depends} on input $i$  %or input $i$  \emph{affects} output $j$ of $f$ 
				if there exists $x,x'\in\{0,1\}^n$ that differ only in the $i$th coordinate such that $f(x)_j\neq f(x')_j$. We say $f$ is $\ell$-local or in the class $\Local^{\ell}$, if every output bit $f_j$ depends on at most $\ell$ input bits. 
			\end{definition}
			
			
			
		
		\subsubsection{Low Depth Circuits and Decision Trees}
		A Boolean circuit with $n$ input bits is a directed acyclic graph in which every node (also called gate) is either an input node of in-degree $0$ labeled by one of the $n$ input bits, an AND gate, an OR gate, or a NOT gate.  One of these gates is designated as the output gate.  The {\em size} of a circuit is its numebr of gates and the {\em depth} of a circuit is the length of its longest path from an input gate to the output gate. 
		
		
		 We consider boolean circuits with unbounded fan-in AND, OR gates everywhere and NOT gates at the input level. We will assume throughout the paper that circuits are {\em alternating}, namely every output gate to input gate path alternates between AND and OR gates. %We also assume the circuits are {\em layered} so that for every gate,
		 We let $\AC_d(S)$ denote alternating depth $d$ circuits of size at most $S$ with unbounded fan-in. For clarity, we take $\AC_d(S,W)$ to denote $\AC_d(S)$ with width at most $W$. Although at small depth, width and size are essentially equivalent: $W\leq S\leq dW$.
		 $w$-$\AC_d(S)$ denotes alternating depth $d$ circuits of size at most $S$ with fan-in at most $w$ at the the first level and unbounded fan-in elsewhere.   For depth $2$ circuits, a DNF is an OR of ANDs (terms) and a CNF is an AND or ORs (clauses). The {\em width} of a DNF (respectively, CNF) is the maximum number of variables that occur in any of its terms (respectively, clauses).  We use $w$-DNF to denote the set of DNFs with width at most $w$.
		 
		 
		 A decision tree with $n$ input bits is a binary tree whose internal nodes have labels from $x_1,\dots,x_n$ and whose leaves have labels from $\zo$. If a node has label $x_i$ then the test performed at that node is to examine the $i$-th bit of the input. If the result is $0$, one descends into the left subtree , whereas if the result is $1$, one descends into the right subtree. The label of the leaf so reached is the output value on that particular input.  The {\em depth} of a decision tree is the number of edges in a longest path from the root to a leaf. Let $\DT(t)$ denote  decision trees with depth at most $t$. 
		 
		 Here are some useful facts relating decision trees and depth $2$ circuits and local functions.  A decision tree of depth $t$ can be computed by a $t$-DNF (respectively $t$-CNF) of size $2^t$ by, for each path associated with a leaf with value $1$ (respectively value $0$), forming a corresponding clause using variables on the path. A boolean function $f$ computed by any depth $t$ decision tree is $2^t$-local because $f$ only depends on variables labeled on the tree and there are at most $2^t$ variables are labeled on a binary tree of depth $t$.
		 
		 $\AC_d(S,W)\circ\DT(t)$ denotes alternating (unbounded fan-in) circuits of depth $d$, size $S$ that take the output of depth $t$ decision trees as input.
		(Note may contain up to $W$ decision trees.)
		Similarly it is helpful to decompose an alternating circuit (from $w-\AC_d$) into a base layer of CNFs or DNFs and the rest of the circuit, $\AC_{d-2}(S,W)\circ w-\AC_2(S')$. (Again, the base may contain up to $W$ CNF/DNFs of size $S'$.)  
		
		
		For a set of boolean circuits $\cC$ (respectively decision trees), we say that a boolean function $f$ is in $\cC$, if there exists a $C\in\cC$ which agrees with $f$ on every input. We say that a multiple output function $f=(f_1,\dots,f_m)$ is in $\cC$ if $f_i\in \cC$ for any $i\in[m]$.
		
		
	
	
		
		
		
	

		


			
		
%		We say $f$ has \emph{output locality} $m$
%		if every output bit $f_j$ is dependent on at most $m$ input bits. 
%		%And $f: \{0,1\}^n \to \{0,1\}^n$ is said to have \emph{input locality} $\ell$,if every input bit affects at most $\ell$ output bits. 
%	%	We say	$f$ is \emph{$(m,\ell)$-local}, $f \in \Local^{m}_{\ell}$,
%	%	if it has input locality $\ell$ and output locality $m$.
%		We denote the class %$\Local^{m}_n$ (namely no restriction on the	input locality) 
%		by $\Local^{m}$. 
%		We say that a bit $x_i$ \emph{affects} the boolean function $f$, \\
%		if $ \, \exists \, \lbrace x_1, x_2, \cdots x_{i-1}, x_{i+1}, \cdots x_n
%		\rbrace \in \zo^{n-1}$ such that, \\
%		$ f(x_1, x_2, \cdots x_{i-1}, 0,
%		x_{i+1}, \cdots x_n) \neq f(x_1, x_2, \cdots x_{i-1}, 1, x_{i+1},
%		\cdots x_n)$.
%
%		Given a function $f=(f_1,\ldots,f_n)$ (where each $f_j$ is a boolean
%		function), we say that input bit $x_i$  \emph{affects} output bit
%		$y_j$, or that output bit $y_j$ \emph{depends} on input bit $x_i$,  if
%		$x_i$ affects $f_j$. 
	

%		\begin{definition}[Output Locality] 
%		  A function $f: \{0,1\}^n \to \{0,1\}^n$ is said to have \emph{output locality} $m$
%		  if every output bit $f_j$ is dependent on at most $m$ input bits.
%		\end{definition}
%
%		\begin{definition}[Input Locality] 
%		  A function $f: \{0,1\}^n \to \{0,1\}^n$ is said to have \emph{input locality} $\ell$
%		  if every input bit affects at most $\ell$ output bits.
%		\end{definition}
%		
%		\begin{definition}[Local Functions]
%		%\Local^{m(n)}_{\ell(n)}
%		  A function $f: \{0,1\}^n \to \{0,1\}^n$ is said to be \emph{$(m,\ell)$-local}, $f \in \Local^{m}_{\ell}$,
%		  if it has input locality $\ell$ and output locality $m$.
%		  We denote the class $\Local^{m}_n$ (namely no restriction on the
%		  input locality) by $\Local^{m}$. 
%		\end{definition}
		
%		\begin{definition}[Leaky-Local]
%			Let $\leaky^{\ell(n),\delta(n),B(n)} \subseteq \{\zo^n \to \zo^n\}$, \emph{Leaky Local $\star$}, denote the set of functions $\{\psi_{f,h,\vb}\}$ where $\psi_{f,h,\vb}(x):=\eval(f(h(x)),x)$ such that
%			\begin{itemize}
%				\item $f$ outputs a circuit 
%				subject to input locality of $x_i$ being bounded by $b_i$,
%				and output locality is at most $\ell(n)$
%				\item $h$ outputs (a fixed set of) $\delta(n)$ bits of $x$
%				\item $\eval([C],x)$ outputs $C(x)$
%				\item $\sum b_i \leq B(n)$
%			\end{itemize}
%		\end{definition}
%		
%		\begin{definition}[Leaky-Local$_\star$]
%			Let $\leaky_\star^{\ell(n),\delta(n),z(n),B(n)} \subseteq \{\zo^n \to \zo^n\}$, \emph{Leaky Local $\star$}, denote the set of functions $\{\psi_{f,h}\}$ where $\psi_{f,h}(x):=\eval(f(h(x)),x)$ such that
%			\begin{itemize}
%				\item $f$ outputs a circuit 
%					subject to input locality of $x_i$ being bounded by $b_i$,
%					and output locality is at most $\ell(n)$
%				\item $h$ is a \emph{depth-$\delta(n)$ decision tree 
%				with leaves over $\zo^{z(n)}$}
%				\item $\eval([C],x)$ outputs $C(x)$
%				\item $\sum b_i \leq B(n)$
%			\end{itemize}
%		\end{definition}
%		
%		\mbnote{Probably remove above Leaky classes definitions.}
%		\sgnote{I agree. I don't really need to use them.}

\subsubsection{Leaky Function Families}
		Given an arbitrary class of tampering functions, we consider a variant of the class of tampering functions which may depend in some limited way on limited leakage from the underlying code word. 
		
		
		\begin{definition} [Leaky Function Families]
		Let $\leaky^{i,m,N}[\cC]$ denote tampering functions generated via the following game:
		\begin{enumerate}
			\item The adversary first commits to $N$ functions from a class $\cC$,
			$F_1,\ldots,F_N = \vF$.
			
			(Note: $F_j:\zo^N\to\zo$ for all $j\in[N]$.) 
			
			\item The adversary then has $i$-adaptive rounds of leakage. In each round $j\in[i]$,
			\begin{itemize}
				\item the adversary selects $s$ indices from $[N]$, denoted $S_j$,
				\item the adversary  receives $\vF(x)_{S_j}$.
				\end{itemize}
				
				Formally, we take $h_j:\zo^{m(j-1)}\to[N]^m$ to be the selection function such that    \[h_j(F(X)_{S_1},\ldots,F(X)_{S_{j-1}})=S_{j}.\]
				Let $h_1$ be the constant function that outputs $S_1$.
				
			\item Finally, selects a sequence of $n$ functions $(F_{t_1},\ldots,F_{t_n})$ ($T=\{t_1,\ldots,t_n\}\subseteq[N]$ such that $t_1<t_2<\cdots<t_n$) to tamper with.
			
				Formally, we take $h:\zo^{mi}\to [N]^n$ such that
				$h(F(X)_{S_1},\ldots,F(X)_{S_i})=T$.
		\end{enumerate}
		Thus, any $\tau\in\leaky^{i,m,N}[\cC]$ can be described as $(\vF,h_1,\cdots,h_i,h)$ and denote the tampering function described above via $\tau = \eval(\vF,h_1,\cdots,h_i,h)$.
		\end{definition}
		

==> put-together.tex <==
\section{Putting It All Together}
In this section, we combine our work in Sections~\ref{sec:bdkm+} and~\ref{sec:ac0-local} to achieve our main results. By composing the non-malleable reductions from Lemma~\ref{lem:ac0} and Lemma~\ref{lem:bdkm}, we obtain a non-malleable reduction which reduces low depth circuit tampering to split state tampering.


\begin{lemma}
\label{lm:ac02ss}
For $S,d,n,\ell\in\bbN$, $p,\delta\in(0,1)$, there exists $\sigma=\poly(\log{\ell}, \log(\ell S),\log(1/\delta),\log(1/p))$ such that for $k$ that $k\geq O(\sigma \log{n})$ and $k=\Omega(n(p/4)^d/\ell^2)$, 	 
	 \[\left(\AC_d(S)\implies\textsc{SS}_{k},d\varepsilon+\exp(-\sigma/2)\right)\] 
where 
	 \[\varepsilon= nS \left(2^{2\log{\ell}+1}(5p\log{\ell})^{\log{\ell}}+ \delta\right) +\exp(-\frac{\sigma}{2\log(1/p)}).\]  
\end{lemma}

For constant-depth polynomial-size circuits (i.e. $\ACZ$), we obtain the following corollary by setting $\ell=n^{1/\log\log\log(n)}$, $\delta=n^{-\log\log(n)}$ and $p=\frac{1}{\log\ell}\cdot \frac{1}{\log n} =\frac{\log\log\log(n)}{\log^2 n}$, 

\begin{corollary}
$\left(\AC0\implies\textsc{SS}_{k},n^{-(\log\log n)^{1-o(1)}}\right)$ for $n=k^{1+o(1)}$. 
\end{corollary}

The same setting of parameters works for depth as large as $\Theta(\log(n)/\log\log(n))$ with $n=k^{1+c}$ where constant $0<c<1$ can be arbitrary small.  We remark that one can improve the error to $n^{-\Omega(\log(n))}$ by using a smaller $p$ value(e.g. $p=n^{-1/100d}$) at the expense of a worse rate (but still $n=k^{1+\epsilon}$).

Combining the non-malleable code for split state from Theorem~\ref{thm:ss-nmc} with rate $1/\log(n)$, we obtain our main theorem.
\begin{theorem}
\label{thm:ac0nmc}
There exists an explicit, efficient, information theoretic non-malleable code for any polynomial-size, constant-depth circuits with error $\negl(n)$ and  encoding length $n=k^{1+o(1)}$.

Moreover, for any constant $c\in(0,1)$, there exists another constant $c'\in(0,1)$ and an explicit, efficient, information theoretic non-malleable code for any polynomial-size, $(c'\log{n}/\log\log{n})$-depth circuits with error $\negl(n)$ and  encoding length $n=k^{1+c}$. 
\end{theorem}


\iffalse

As a byproduct, by combing Lemma~\ref{lem:bdkm} with Theorem~\ref{thm:ss-nmc}, we obtain non-malleable codes for leaky local functions  which may be of independent interest.

\begin{corollary}
	\label{lem:local-nmc}
	If $(\E_{\text{SS}},\D_{\text{SS}})$ is an explicit, efficient, information theoretic $(\text{SS},\epsilon)$-non-malleable code with relative rate $R(k)$, $R(k)=k/n$,
	
	then there is an explicit, efficient information theoretic $(\leaky^{k,m,N}[\Local^\ell],\exp(-\Omega(\sigma))+\epsilon)$-non-malleable code with codewords of length $n=O(\ell^2(k/R(k)+mq\ell+s(\sigma))$.
	
	In particular, assuming a $(\text{SS},\exp(-\Omega(k)))$-non-malleable code with $R(k)=\Omega(1/\log n)$ (as in~\cite{Li17}):
	\begin{enumerate}
		\item For $\gamma<1/3$, $mq \leq n^{(1-3\gamma)}$, and $\ell\leq n^{\gamma}$,
		there is an explicit, efficient, information theoretic $(\leaky^{k,m,N}[\Local^{\ell}],\exp(-\Omega(k)))$-non-malleable code.
		
		Moreover, the rate can be made \emph{almost} linear: 
		for $n=O(k^{1+\delta})$ $(\delta>0)$,
		take $\gamma < \frac{\delta}{2(1+\delta)}(\approx \frac{\delta}{2})$.
		%k^{1+\delta}=n \iff n^{1/(1+\delta)}=k
		%\iff 1/(1+\delta) = 1-2\eps
		%\iff 1 = (1-2\eps)(1+\delta)
		%\iff 1 = 1 - 2\eps +\delta -2\eps\delta
		%\iff \delta = 2\eps(1+\delta)
		%\iff \eps = \delta/(2+2\delta)
		%and then an extra factor of log k, handle by shaving exponent
		\item For
		$mq\ell^3=o(n)$ and ($\sigma=\theta(k)$),
		$(\leaky^{k,m,N}[\Local^\ell],\exp(-\Omega(k)))$ with rate $\Omega(\frac{1}{\ell^2\log n})$.
		In particular, for $\ell=\tilde{O}(1)$ the code has quasilinear rate.		
	\end{enumerate}
\end{corollary}
\fi

%\mbnote{fill in what is needed for cor: composition + \cite{Li17}.}
%\dnote{Do we actually get security $\exp(-\Omega(k))$? I think the security will depend on the
%	$\sigma$ of the $\sigma$-wise independent generator. 
%	See argument that $H_0\approx_{\negl(n)} H_1$ below.
%	Are you saying that $\sigma$ can be as large as
%	$\Omega(k)$? Or should we think of $\sigma$ as $polylog(k)$?}


==> reduction.tex <==
In this section, we define a simple encoding and decoding scheme based on the pseudorandom switching lemma. To illustrate the rational behind our choices and the power of the scheme, we show this scheme is a non-malleable reduction from class $\mathcal{F}$ to class $\mathcal{G}$ with limited leakage if functions in $\mathcal{F}$ reduce to $\mathcal{G}$ under pseudorandom restrictions. 


\begin{proposition}\label{prop:psl-nmr}
	Let $\mathcal{F} \subset A^A$ and $\mathcal{G} \subset B^B$ be some classes of functions  where $A=\zo^n$ and $B=\zo^k$. Let $\cD$ be any $\sigma$-wise independent distribution over $\zo^{n\log(1/p)}\times\zo^n$.
	If for any $f\in\mathcal{F}$, 
	\[\Pr_{\rho\gets\cR(\cD)}\left[ F_\rho \text{ is not in } \mathcal{G}\right]
	\leq \varepsilon,\]
	then $(\E^\star,\D^\star)$ defined in figure~\ref{fig:red}, is an $(\mathcal{F}\implies\leaky^{1,m,n}[\mathcal{G}],\varepsilon+\exp(-\Omega(\frac{\sigma}{\log(1/p)}))$-non-malleable reduction with rate $\Omega(1/p)$ where $m=O(\sigma\log n)$.
\end{proposition}

\iffalse
\begin{proposition}\label{prop:DNF}
	For  $w,\ell\in \bbN$, $(\E^\star,\D^\star)$ defined in figure~\ref{fig:red}, is a $(w$-$\mathrm{DNF}\implies\leaky^{1,m,n}[\Local^{\ell}],\varepsilon)$-non-malleable reduction where $\sigma=\poly(\log l,w,\log(1/\delta),\log(n))$, $m=O(\sigma\log(n))$ and $\varepsilon\leq \exp(-\sigma/2) + n\left(2^{w+\log\ell+1}(5pw)^{\log \ell}+ \delta\right)$.  
%		\item $\rho$ is independent of $x$,
%		\item The probability that $\zeta'$ is used (or, $L(G(\zeta))$ doesn't have enough $1$s) is $<\exp(-q/2)$,
		%\mu = 2^{-\log(1/p)}(n-m)\geq p/3 n \geq 2k
%		\item $\Pr[\D^*(\E^*(x))=x]=1$.
\end{proposition}
\fi

\iffalse
As an example, by choosing $q=\poly(\log(n))$, $p=1/\log^2(n)$, and combining with Lemma~\ref{lem:psl}, $(\E^\star,\D^\star)$ is a non-malleable reduction from width-$O(\log(n))$ DNFs to $\leaky^{1,m,n}[\Local^{k^{\Omega(1)}}]$ with $\negl(n)$ error. In addition the rate is $\Omega(p)=\Omega(1/\log^2{n})$ and the leakage is $m=\poly(\log(n))$.

%\sgnote{These paragraphs in below can be moved to the intro or removed.}


Let us illustrate the intuition behind the scheme. For concretenss, let us focus on the case that $\mathcal{F}$ is the family of width-$w$ DNFs and $\mathcal{G}$ is the family of local functions. Recall that by the definition of non-malleable reduction,  $(\E^\star,\D^\star)$ needs to satisfy two conditions (i) $\Pr[\D^\star(\E^\star(x))=x]=1$ for any $x$ and, (ii) $\D^\star\circ f\circ \E^\star$ is a distribution over (leaky) local functions for any width-$w$ DNF $f$.  

%\sgnote{Why random restriction and why it doesn't work} 
It is well known that, by switching lemma, DNFs become local functions under random restrictions. Therefore towards satisfying (ii), a natural choice of $\E^\star$ is simply generating a random restriction and embedding the message in star locations. However, although $f\circ \E^\star$ becomes local, $\D^\star$ doesn't know star locations thus fails (i). To satisfy (i), the naive idea is to append the star location information in the encoding. However, now we cannot use random restrictions to reduce DNFs to local functions because of the dependences.

%\sgnote{Why pseudorandom restriction and RPE}
To circumvent those limitations, the main idea is to employ pseudorandom switching lemma by Trevisan and Xue~\cite{TX13}, which reduces DNFs to local functions while only requires limited dependence from the underlying restriction. In particular, we append an encoding of the seed $\zeta'$ of the restriction  into the restriction so that, we can decode $\zeta'$ later and the overall restriction is sufficient to make DNFs  local. More specifically, we encode $\zeta'$ using RPE whose privacy property guarantees that the overall restriction is $\sigma$-wise independent and the decoding property enables us to decode $\zeta'$.  


%\sgnote{Why leaky local}
Up to this point, we can satisfy (i) easily:  $\D^{\star}$ decodes $\zeta'$ from the encoded $\zeta'$ (say always in the first $m'$ coordinates), then figuring out the star locations and extracting the message from the star locations. In addition, $f\circ \E^\star$ becomes a distribution over local functions where the distribution only depends on $f$ (not the message). However, composing $\D^\star$ with $f\circ \E^\star$ induces dependence on underlying message: tampered encoding of $\zeta'$, may depend on the message in the star locations. In order to simulate $\D^\star$ with $f\circ \E^\star$, we choose to work with the class of leaky local functions which allow one to obtain limited number of local functions computed on underlying message then choose other local functions to be the tampering function. This class enables us to first obtain the tampered encoding of the seed, then output a tampering local function which doesn't depend on the message.  

%\sgnote{Why $q$-wise independent generator} 
Up to here, we get a non-malleable reduction which reduces DNFs to leaky local where roughly $m'=|\E_{R}(\zeta')|$ local functions need to be leaked.  $m'$ can be as long as the entire message so there may not exist any non-malleable code for leaky local functions with such leakage. To minimize the amount of needed leakage, we derandomize $\zeta'$ using a bounded-wise independence generator $G$ with a much shorter seed $\zeta$ and then store the encoding of $\zeta$ instead. %Fortunately, pseudorandom switching lemma still works as before and overall we get a non-malleable reduction for DNFs to leaky local functions where only $m=|\E_{R}(\zeta)|$ functions need to be leaked.
\fi

 The proposition immediately follows from  Claim~\ref{cl:correctness}, Claim~\ref{cl:simulation} and Claim~\ref{cl:error}.
\begin{claim} \label{cl:correctness}
For any $x\in\zo^{k}$, $\Pr[\D^*(\E^*(x))=x]=1$.
\end{claim}
\begin{proof}
The second step of $\E^*$ guarantees that $\extInd(L(G(\zeta)))_1>m$ and $\|L(G(\zeta)\|_0\geq k$. Therefore, $\E_R(\zeta)$ is located in the first $m$ bits of $c$ and the entire $x$ is embedded inside the remaining $n-m$ bits of $c$ according to $L(G(\zeta))$. By the decoding property of RPE from lemma~\ref{lem:rpe}, $\Pr[\D_R(c,\dots,c_m)=\zeta]=1$, namely, $\Pr[\tilde{\zeta}=\zeta]=1$. Conditioned on $\tilde{\zeta}=\zeta$, because $\|L(G(\zeta)\|_0\geq k$, $\D^{*}(\E^*(x))=\extract(c,L(G(\zeta)))=x$ holds. The desired conclusion follows.
\end{proof}


\begin{claim} \label{cl:simulation}
For any $F\in\mathcal{F}$, there exists a distribution $\mathcal{H}$ over functions in $\leaky^{1,m,n}[\mathcal{G}]$ such that for any $x\in\zo^k$,   $\mathcal{H}(x)$ is $\delta$-close to  $(\D^*\circ f\circ\E^*)(x)$ where $\delta\leq \Pr[\text{$f\circ\E^*$ is not in $\mathcal{G}$}]$.
\end{claim}
\begin{proof}  Recall that a function $\tau$ in $\leaky^{1,m,n}[\mathcal{G}]$ can be described as $(\vF,h_1,h)$ where $\vF$ is a function in $\mathcal{G}$ from $\zo^k$ to $\zo^n$, $h_1$ is a contant function outputs a set $S_1$ of size $m$, and for every $x\in\zo^k$, $h$ takes $\vF(x)_{S_1}$ as input and outputs a set $T$ of size $k$. And the evaluation of $\tau$ on $x$ is $\vF(x)_T$.  
	
Fix an arbitrary $f\in\mathcal{F}$.  We define $\mathcal{H}$ over $(\vF,h_1,h)\in \leaky^{1,m,n}[\mathcal{G}]$ as follows.  $\mathcal{H}$ samples a function $\vF$ from the distribution $f\circ\E^{*}$ by sampling $\zeta, U$, generating $\rho$ and setting $\vF = f_{\rho}$, if $\vF$ is not in $\mathcal{G}$, let $\vF$ be some fixed constant function; $h_1$ always outputs $[m]$; finally, for every $x\in\zo^n$, $h$ takes $\vF(x)_{[m]}$ as input and outputs $T=\extInd(L(G(\D_R(\vF(x)_{[m]}))))$ . 
	
Fix any $x\in\zo^k$. For any choice of $(\zeta,U)$ so that $f\circ\E^{*}(\cdot;\zeta,U)$ is in $\mathcal{G}$, note that $\vF(x)_T$ is exactly $\D^{*}\circ f\circ\E^{*}(x)$, in other words,  $\D^{*}\circ f\circ\E^{*}(x;\zeta,U)=\mathcal{H}(x;\zeta,U)$ holds. Hence the distance between $\D^{*}\circ f\circ\E^{*}(x)$ and $\mathcal{H}(x)$ is at most $\Pr[\text{$f\circ\E^*$ is not in $\mathcal{G}$}]$.
\end{proof}


\begin{claim} 	\label{cl:error} 
For any $f\in\mathcal{F}$, $\Pr[\text{$f\circ\E^*$ is not in $\mathcal{G}$}]\leq \varepsilon + \exp(-\Omega(\frac{\sigma}{\log(1/p)})$.
%	$f\circ\E^*$ is not $\ell$-local with probability at most $M\left(2^{w+\log\ell+1}(5pw)^{\log \ell}+ \delta\right)$ over the randomness of $\E^*$.
\end{claim}
\begin{proof}
We first show $\cD=G(\zeta)\|\E_R(\zeta)\|U$ is $\sigma$-wise independent when $\zeta\gets\{0,1\}^s$ and $U\gets\{0,1\}^{n-m}$.  As $U$ is uniform and independent of the rest, it suffices to simply consider $Z=G(\zeta)\|\E_R(\zeta)$.
Fix some $S\subseteq [n\log(1/p)+m]$ such that $|S|\leq \sigma$.
By the secrecy property of the RPE and  $m\cdot\csec\geq \sigma$, conditioned on any fixed $\zeta$, $Z_{S\cap\{n\log(1/p)+1,\ldots,n\log(1/p)+m\}}$is distributed uniformly.
Therefore, $\zeta$ is independent of $Z_{S\cap\{n\log(1/p)+1,\ldots,n\log(1/p)+m\}}$, so $G$ guarantees that $Z_{S\cap\{1,\ldots,n\log(1/p)\}}$ is also distributed uniformly and independently of ${S\cap\{n\log(1/p)+1,\ldots,n\log(1/p)+m\}}$.
Therefore, $Z_S$ is distributed uniformly.

Note that $\rho$ in $\E^{*}$ distributes the same as $\cR(\cD)$ except when $\zeta^{*}$ is used.  Hence 
\[\Pr[\text{$f\circ\E^*$ is not in $\mathcal{G}$}] \leq \Pr_{\rho\gets\cR(\cD)}\left[ F_{\rho} \text{ is not in } \mathcal{G}\right]+\Pr[\|L(G(\zeta))_{n-m+1,\ldots,n}\|_0<k].\]
Because $\cD$ is $\sigma$-wise independent, $\Pr_{\rho\gets\cR(\cD)}\left[ F_{\rho} \text{ is not in } \mathcal{G}\right]\leq \varepsilon$. Observe that $L(G(\zeta))_{n-m+1,\ldots,n}$ is a $\frac{\sigma}{\log(1/p)}$-wise independent distribution over $\zo^{n-m}$ that so each coordinate is $1$  with probability $1/p$. By Theorem~\ref{thm:pr-chernoff} and our choice of parameter satisfying that $\mu:=(n-m)p\geq 2k$ and $\frac{\sigma}{\log(1/p)}\leq (1/2)^2 \mu e^{-1/3}$, $\|L(G(\zeta))_{n-m+1,\ldots,n}\|_0<\mu/2$ happens with probability at most $\exp(-\Omega(\sigma/\log(1/p))$. The desired conclusion follows.

	

\end{proof}








	
\begin{figure}[ht!]
		\fbox{\parbox{\textwidth}{
				
				\small \center
				\begin{minipage}{0.95\textwidth}
					Take  $k,n,p,\sigma$ to be parameters (such that $np\geq 4k$, $k\geq 4\sigma$, $n\geq 10\sigma\log(n)$).
					\mbnote{I'm not sure I undertand these constraints entirely (we can state the chernoff bounds more generally, if that is the issue)
					$p(n-m(\sigma)\geq 2k$, $m(\sigma)\geq \crate s(\sigma)=\crate \sigma \log n$ (because $pn>1$ and hence $\log 1/p \leq \log n$)}
						
					Let $G_{\sigma}\colon\zo^{s(\sigma)}\to\zo^{n\log1/p}$ be an $\sigma$-wise independent generator
					from lemma~\ref{lem:gen}. %where $s=(q+1)\log(n\log(1/p))$.
						
					Let $(\E_R,\D_R,\R_R)$ denote the RPE from lemma~\ref{lem:rpe} with codewords of length $m(s)\geq \sigma/\csec$.
						
					Let $\zeta^*\in\zo^{s(\sigma)}$ be some fixed string such that $\|L(G(\zeta^*))_{n-m+1,\ldots,n}\|_0\geq k$. %For $G$ from Lemma~\ref{lem:gen} such a $\zeta'$ can be found via interpolation in time $O(q\log^2n)$.
					
					
					\begin{itemize}
						\item[]{\bf $\E^\star(x)$:}
						
						\begin{enumerate}
							\item Draw (uniformly) random seed $\zeta\gets\{0,1\}^s$ 
							and (uniformly) random string $U\gets\{0,1\}^{n-m}$.
							
							\item Generate pseudorandom restriction, $\rho=(\rho^{(1)},\rho^{(2)})$:
							\begin{itemize}
								\item[] $\rho^{(1)} \gets L(G(\zeta))$;
									($*$) If $\|L(G(\zeta))_{n-m+1,\ldots,n}\|_0< k$, set $\zeta=\zeta^{*}$. 
								
								\item[] $\rho^{(2)} \gets \E_R(\zeta)\|U$.
							\end{itemize}
							
							\item Output $c=\embed(x,\rho)$.
						%	\mbnote{change description to $\extInd$ (match $S$) for clarity}
						\end{enumerate}
						
					
						% $L(G(\zeta))$ is $\leq n-m$
						% (or does not exist).
						
						
						\item[]{\bf $\D^\star(\tilde{c})$:}
						\begin{enumerate}
							\item Recover tampered seed: 
							$\tilde{\zeta}\gets\D_R(\tilde{c}_1,\ldots,\tilde{c}_m)$.
							
							If $\|L(G(\tilde{\zeta}))\|_0<k$ or $\extInd\big(L(G(\tilde{\zeta}))\big)_1\leq m$, output $\bot$ and halt.
							\item Output
							$\extract\big(\tilde{c},L(G(\tilde{\zeta}))\big)$.
						\end{enumerate}
					\end{itemize}
					\medskip
				\end{minipage}}}
				\caption{A Pseudorandom Restriction Based Non-Malleable Reduction, $(\E^\star_{k,n,p,\sigma},\D^\star_{k,n, p, \sigma})$}
				\label{fig:red}
			\end{figure}

\iffalse
	We now define a simple encoding scheme that embeds a message in a pseudorandom restriction such that it can be later extracted.


\begin{proposition}
	\label{prop:red}
	The reduction from figure~\ref{fig:red} has the following properties.
\begin{enumerate}
	\item $s=(q+1)\log(n\log 1/p)$,
	\item $m=\crate s\geq q/\csec$ (for $n$ large enough),
	\item $\rho$ is independent of $x$,
	\item The probability that $\zeta'$ is used (or, $L(G(\zeta))$ doesn't have enough $1$s) is $<\exp(-q/2)$,
	%\mu = 2^{-\log(1/p)}(n-m)\geq p/3 n \geq 2k
	\item $\Pr[\D^*(\E^*(x))=x]=1$.
\end{enumerate}
\end{proposition}
The above can be verified by inspection.
\sgnote{maybe we draw another picture to make it more clear}
\mbnote{yeah?}

Additionally, we show that the $\rho$ generated in steps 1 and 2 (independently of the message $x$), is $q$-wise independent.
	\begin{lemma}
		\label{lem:ind}
		$G(\zeta)\|\E_R(\zeta)\|R$ generated as in steps 1 and 2 of $\E^\star$ is $q$-wise independent.
	\end{lemma}
	\begin{proof}
		As $R$ is uniform and independent of the rest, it suffices to simply consider $Z=G(\zeta)\|\E_R(\zeta)$.
		Fix some $S\subseteq [n\log(1/p)+m]$ such that $|S|\leq q$.
		By the secrecy property of the RPE,
		conditioned on any fixed $\zeta$, $Z_{S\cap\{n\log(1/p)+1,\ldots,n\log(1/p)+m\}}$ is distributed uniformly.
		Therefore, $\zeta$ is independent of $Z_{S\cap\{n\log(1/p)+1,\ldots,n\log(1/p)+m\}}$, so $G$ guarantees that $Z_{S\cap\{1,\ldots,n\log(1/p)\}}$ is also distributed uniformly and independently of ${S\cap\{n\log(1/p)+1,\ldots,n\log(1/p)+m\}}$.
		Therefore, $Z_S$ is distributed uniformly.
	\end{proof}
	
	
\fi

==> siyao_intro.tex <==
\section{SiyaoIntroTry}
Non-malleable codes were first introduced by Dziembowski, Pietrazak and Wichs~\cite{DPW10} as an elegant extension of error-correcting codes which aim to handle a much larger class of tampering functions than the traditional error-correcting codes.  Unlike error-correcting codes which gurantee correct decoding of corrupted codewords, non-malleable codes instead guarantee that the decoding is either correct or independent of the orginal message. Informally, given a tampering function family $\mathcal{F}$, an $\mathcal{F}$-non-malleale code $(\E,\D)$ encodes a given message $x$ in a way such that if the codeword $y\leftarrow\E(x)$ is modified into $y'=f(y)$ by some $f\in\mathcal{F}$, then the decoded message $x'=\D(y')$ is either the originial message or is a completely unrelated value. 

As shown by~\cite{DPW10}, this relaxation makes non-malleable codes quite useful in a variety of situations where tranditional error-correcting (even error-detection code) is impossible: a) the tampering capabilities of the attacker are too strong for error-detection; b) changing the secret to unrelated secret is not useful for the attack. For example, imagine $x$ being a secret key for a signature scheme. Because tampering $x$ to unrelated $x'$ is not useful in forging signatures under the originial (un-tampered) verification key, encoding $x$ under non-malleable code will provide meaningful message integrity. Besides the straighforward tamper-resislient application, non-malleable codes (and its later variants) have been found unexpected applications in cryptography such as constructing non-malleable encryptions~\cite{CMTV15,CDTV16} and giving extremely simple 3-round optimal non-malleable commitments~\cite{GPR16}.
%Moreoever, non-malleable codes have been found to have a connection with various types of randomness extractors~\cite{DKO13,CG14a} which allow one to harness deep theorems from the extensive randomness extraction literature to cyrptography. 


What tampering class can efficient non-malleable code handle? Unfortunately, as pointed out by~\cite{DPW10}, it is impossible to constructing efficient codes secure against arbitrary polynomial time tampering adversary, since the adversary can apply a tampering function that decodes the entire codeword to recover the mseegae $x$ then re-encode a related message. %At the same time, for any function family of size at most $2^{2^{\alpha n}}$, there exists inefficient non-malleable code with rate $1-\alpha$.
To bypass this limitation, besides non-explict and inefficient constructions, almost all prior work considered restricted tampering classes where each output of the function only depends on a subset of the input, including bit-wise temparing~\cite{DPW10,CKM11,CCFP11}, split-state~\cite{LL12,DKO13,ADL14,CG14a,CG14b,ADKO15,Li17}, constant split-state~\cite{CZ14}, permutations~\cite{AGMPP15a,AGMPP15b}, and local functions~\cite{BDKM16}. The only exception is the recent work by Chattopadhyay and Li~\cite{CL17} which builds a non-malleable code for $\ACZ$, the class of constant depth, polynomial size circuits. However, to encode a $k$-bit message, the codeword requires $2^{O(\sqrt{k})}$ length. Hence, prior to our work, the following question remained open: 
\begin{quote}
	Can we construct efficient, information theoretically secure non-malleable codes against $\ACZ$ with $\poly(k)$-bit long codeword for a $k$-bit message?
\end{quote}

\subsection{Our Results}
In this work, we resolve this open problem. 
\begin{theorem} 
	For any $k$ and $\varepsilon$, there exists an efficient (in $k$ and $\log(1/\varepsilon)$) information-theoretically secure $\varepsilon$-non-malleable code for $\AC_d(S)$, encoding $k$-bit messages into a string of length $n=k^{1+\gamma}$ bits. The encoding and decoding run in time polynomial in $k$.
\end{theorem}

For constant-depth circuits of polynomial-size (i.e. $\ACZ$ tampering functions), our codes have cordword length $n = k^{1+o(1)}$ for a $k$-bit message, which is an exponential improvement of the previous best construction~\cite{CL17} (which had codeword length $2^{O(\sqrt{k})}$). Our construction remains efficient for circuit depths as large as $\Theta(\log(n)/\log\log(n))$ and the  codeword length remains $\leq k^{1+\varepsilon})$. 
Extending our result beyond $\log(n)/\log\log(n)$ depth will give a non-malleable code for logrithmic-depth polynomial-size circuits with bounded fan-in gates (i.e. NC1) thus separating NC1 from P (note there is no non-malleable code for P~\cite{DPW10}). 


We remark that the originial work of~\cite{DPW10} (and the improvement in~\cite{CG14a}) gives existential result of non-malleable codes against $\ACZ$ (thus inefficient encoding and decoding) and some work gives conditional non-malleable codes.   Our work gives explicit, unconditional construction.




\subsection{Our Approach}
To prove our results, we use the concept of {\em non-malleable reudctions}, introduced by Aggarwal et al.~\cite{ADKO15}. Loosely speaking, a class of functions $\mathcal{F}$ reduces to the class $\mathcal{G}$, if there is a pair of encoding and decoding algorithms $(\E,\D)$ satisfying that for any $f\in\mathcal{F}$, there is a distribution $G_f$ over functions in $\mathcal{G}$ such that for every $x$, $\D(f(\E(x)))$ and $G_f(x)$ are statistically close. \cite{ADKO15} showed that a non-malleable code for $\mathcal{G}$ can be used to construct one for $\mathcal{F}$, and provide an elegant and powerful composition theorem for constructing non-malleable codes.  

Following this technique, we obtain our main result by reducing low depth circuits to split state then compose this reduction with known results for split state functions. As an intermediate step, we consider a variant of local functions which we call leaky local functions. And we prove two reductions, one reduces low depth circuits to leaky local functions and the other one reduces leaky local function to split state. 

\paragraph{Low Depth Circuits to Local Functions.}
Let us first show how to reduce depth $2$ circuits to the family of local functions. A non-malleable reduction  $(\E,\D)$ reducing $\mathcal{F}$ to $\mathcal{G}$ needs to satisfy two conditions (i) $\Pr[\D(\E(x))=x]=1$ for any $x$ and, (ii) $\D\circ f\circ \E$ is a distribution over (leaky) local functions for any width-$w$ DNF $f$.  It is well known that, by switching lemma, DNFs become local functions under random restrictions. Therefore towards satisfying (ii), a natural choice of $\E$ is simply generating a random restriction and embedding the message in star locations. However, although $f\circ \E$ becomes local, $\D$ doesn't know star locations thus fails (i). To satisfy (i), the naive idea is to append the star location information in the encoding. However, now we cannot use random restrictions to reduce DNFs to local functions because of the dependences.

To circumvent those limitations, the main idea is to employ {\em pseudorandom switching lemma} by Trevisan and Xue~\cite{TX13}, which reduces DNFs to local functions while only requires limited dependence from the underlying restriction. In particular, we append an encoding of the seed $\zeta'$ of the restriction  into the restriction so that, we can decode $\zeta'$ later and the overall restriction is sufficient to make DNFs  local. More specifically, we encode $\zeta'$ using RPE whose privacy property guarantees that the overall restriction is $\sigma$-wise independent and the decoding property enables us to decode $\zeta'$.  


%\sgnote{Why leaky local}
Up to this point, we can satisfy (i) easily:  $\D$ decodes $\zeta'$ from the encoded $\zeta'$ (say always in the first $m'$ coordinates), then figuring out the star locations and extracting the message from the star locations. In addition, $f\circ \E$ becomes a distribution over local functions where the distribution only depends on $f$ (not the message). However, composing $\D$ with $f\circ \E$ induces dependence on underlying message: tampered encoding of $\zeta'$, may depend on the message in the star locations. In order to simulate $\D$ with $f\circ \E$, we choose to work with the class of leaky local functions which allow one to obtain limited number of local functions computed on underlying message then choose other local functions to be the tampering function. This class enables us to first obtain the tampered encoding of the seed, then output a tampering local function which doesn't depend on the message.  

%\sgnote{Why $q$-wise independent generator} 
Up to here, we get a non-malleable reduction which reduces DNFs to leaky local where roughly $m'=|\E_{R}(\zeta')|$ local functions need to be leaked.  $m'$ can be as long as the entire message so there may not exist any non-malleable code for leaky local functions with such leakage. To minimize the amount of needed leakage, we derandomize $\zeta'$ using a bounded-wise independence generator $G$ with a much shorter seed $\zeta$ and then store the encoding of $\zeta$ instead.

To deal with depth $d$, we simply apply the this restriction $d$ times and trade depth for leakage.

\paragraph{Leaky Local Functions to Split State.}
Ball et al.~\cite{BDKM16} gave a non-malleable code for local functions via a non-malleable reduction to split state. We revisit their reduction and show leaky local functions can be reduced to split state. Because previous reduction can reduce low depth circuits to $\ell$-local for $\ell=k^c$ for an arbitrary small constant $c<1$, it suffices for us to adapt a simple reduction from the appendix of \cite{BDKM16}.  This reduction is relative simple and doesn't use randomized decoding.


%\paragraph{Organization of this Paper.} 
%In Section~\ref{sec:preliminaries}, we define conventions, non-malleable codes and tampering classes. In Section~\ref{sec:ingredients}, we give the basic ingredients in our paper. In Section~\ref{sec:reduction} and~\ref{sec:leaky}, we reduce $\AC_d(S)$ to leaky local functions and in the last section we reduce leaky local functions to split state model.

==> wDNF.tex <==
	\begin{figure}[ht!]
		\fbox{\parbox{\textwidth}{
 
		\small \center
		\begin{minipage}{0.95\textwidth}
			Let $\ell=???,B=???,\delta=???$.
	Let $(\E_R,\D_R,\R_R)$ denote the RPE from lemma~\ref{lem:rpe} with codewords of length $m(s)=???$.
	Let $(\E_\ell,\D_\ell)$ denote the NMC against $\leaky^{\ell,\delta,B}$ corollary~\ref{cor:bdkm16}.
	Let $G(s)$ be an $q$-wise independent generator.
	\begin{itemize}
		\item[]{\bf $\E(x)$:}
		\begin{enumerate}
			\item Draw random seed $\zeta\gets\{0,1\}^s$ and random string $r\gets\{0,1\}^{N-m}$.
			\item Use $L(G(s))$ to generate $\rho_\star$.
			\mbnote{clarify}
			\item Let $c_1 = \E_R(\zeta)$
			\item Let $c_2$ denote the result of embedding $x$ in $r$ according to $\star$s in the last $k$ locations of $\rho_\star$.
			\mbnote{clarify}
			\item Output $c_1,c_2$
		\end{enumerate}
		
		\item[]{\bf $\D(\tilde{c}_1,\tilde{c}_2)$:}
		\begin{enumerate}
			\item Decode tampered seed: 
			$\tilde{\zeta}\gets\D_R(\tilde{c}_1)$.
			\item Get tampered locations, $\tilde{\rho}_\star$ via 
			$L(G(\tilde{\zeta}))$
			\item Output the bits corresponding to the last $k$ indices with $\star$ in $\tilde{\rho}_\star$.
		\end{enumerate}
	\end{itemize}
	\medskip
	\end{minipage}}}
	\caption{A Non-Malleable Reduction $(\dnf \implies \leaky)$}
	\end{figure}
	
	\begin{theorem}
		$(\E,\D)$ is a $(w\mbox{-}\dnf \implies \leaky^{\ell,\delta,B})$-non-malleable reduction.
	\end{theorem}
	
	\begin{proof}
	We begin by describing a simulator that outputs $\leaky$ tampering, independent of the message.
	Then, we demonstrate that with overwhelming probability real tampering composed with the reduction is identical to the simulated tampering. This follows from an application of Lemma~\ref{lem:psl}.
	
	\begin{figure}[ht!]
		\fbox{\parbox{\textwidth}{

		\small \center
		\begin{minipage}{0.95\textwidth}
	given $\ACZ$ tampering $\tau$ outputs $\psi_{f,h,b}$ as follows:
	\begin{enumerate}
	\item Sample $\zeta,r$ as in $\E$.
	\item Encode seed: $\E_R(\zeta)=c_1$
	\item Generate random restriction $\rho$ %$=(\rho_{\bar{\star}},\rho_\star)$
	 where $\rho_{\bar{\star}}=c_1\|r$ and $\rho_\star$ is generated from $L(G(\zeta))$ as in $\E$.
	Let $L_1,\ldots,L_k$ denote the last $k$ indices of $L(G(\zeta))$.
	
	If $L_1<n-m$ or $k$ such indices do not exist, output some constant function.
	\item Apply (constructive) switching lemma with pseudorandom restriction to get $\Local^\ell$ function $t':=\tau|_\rho$ ($n$-bit output).
	
	If not all circuits collapse to $\ell$-local functions, halt and output some constant function.
	
	Fix bounds on input locality $\vb=(b_{L_1},\ldots,b_{L_n})$ according to the output local function $t$.
	\item Let $t:=t'$ where any input bits originally drawn from $[m]$ are fixed to the corresponding value in $c_1$.
	\item The function $h$ outputs the (at most) $\ell \cdot m$ (uniformly chosen bits) corresponding to locations with $\star$'s (according to $\rho_\star$) in the last $n$ locations that effect the functions $t_1,\ldots,t_m$.
	(Note that $t_1,\ldots,t_m$ only depend on the output of $h$.)
	\item Output the following function $f$, which has $t_1,\ldots,t_n$ hardcoded, and that on input $h(x)$
	\begin{enumerate}
		\item Get $\hat{\zeta}$ by evaluating $t_1,\ldots,t_m$ on $\E(\zeta)$ and $h(x)$
		\item Expand $\hat\zeta$ via $G$ to get (tampered) decoding locations: $\hat{i}_1,\ldots,\hat{i}_m$
		\item Output (local) functions $t_{i_1},\ldots,t_{i_k}$.
	\end{enumerate}
	\item Finally, output $\psi_{f,h,b}$.
	\end{enumerate}
	\medskip
	\end{minipage}}}
	\caption{Simulator, $\Sim$, for $(\E,\D)$}
	\end{figure}
	
	\begin{claim}
		\label{clm:ind}
		For $\crate \cdot m > q$ uniformly drawn $\zeta$,
		$Z=\E_r(\zeta)\|G(\zeta)$
		is $q$-wise independent.
	\end{claim}
	\begin{proof}
		Fix some $S\subseteq [m+N\log(1/p)]$ such that $|S|\leq q$.
		By the secrecy property of the RPE,
		conditioned on any fixed $\zeta$, $Z_{S\cap[m]}$ is distributed uniformly.
		Therefore, $\zeta$ is independent of $Z_{S\cap[m]}$, so $G$ guarantees that $Z_{S\cap\{m+1,\ldots,N\log(1/p)\}}$ is also distributed uniformly and independently of $Z_{S\cap[m]}$.
		Therefore, $Z_S$ is distributed uniformly.
	\end{proof}
	
	This very simple claim allows us to apply the pseudorandom switching lemma, Lemma~\ref{lem:psl}, and prove the following:
	\begin{claim}
		$\forall \tau \in w\mbox{-}\dnf$, $\forall x\in\cC$ (the set of $leaky$-non-malleable codewords)
		\[\Delta(\D(\tau(\E(x)));\Sim_\tau(x))\leq ???.\]
	\end{claim}
	\begin{proof}
		
		Notice that the random restriction $\rho$ where only the last $k$ locations survive is distributed identically to $\E(*\cdots*)$ (encodings of all star messages). \mbnote{this is technically not defined.} In other words, both the simulator and encoder use randomness identically.
		Fix randomness $\zeta,r$ and $r'$, the randomness of $\E_R$.
		This in turn fixes a random restriction $\rho$.
		
		Let $E$ denote the event that
		\begin{enumerate}
			\item for all $i\in[n]$,
			$\tau_i$ is equivalent to an $\ell$-local function after applying a random restriction sampled as in $\Sim$,
			\item the random restriction contains at least $k$ survivors in the last $n-m$ locations.
		\end{enumerate}
		By Lemma~\ref{lem:psl} and Claim~\ref{clm:ind},
		we know the that $E$ happens with probability at most ???.
		\mbnote{Additionally add that all $\dnf$ of width more than $w$ are constant (and change theorem statement).}
		
		Moreover, for fixed randomness $\zeta,r$ and $r'$, the randomness of $\E_R$, which in turn fixes a random restriction $\rho$, the resulting tampering is identical (and resulting function) only depends on $x$.
		(This can be verified by inspection.)
		
		Thus, the distributions are identical conditioned on $E$ not occurring.
		Therefore, the statistical difference of the two distributions is at most ???.
	\end{proof}
	\end{proof}
	
